InnovationInsights: A Visual Analytics Approach for Understanding the Dual Frontiers of Science and Technology

Science has long been viewed as a key driver of economic growth and rising standards of living. Knowledge about how scientific advances support marketplace inventions is therefore essential for understanding the role of science in propelling real-world applications and technological progress. The increasing availability of large-scale datasets tracing scientific publications and patented inventions and the complex interactions among them offers us new opportunities to explore the evolving dual frontiers of science and technology at an unprecedented level of scale and detail. However, we lack suitable visual analytics approaches to analyze such complex interactions effectively. Here we introduce InnovationInsights, an interactive visual analysis system for researchers, research institutions, and policymakers to explore the complex linkages between science and technology, and to identify critical innovations, inventors, and potential partners. The system first identifies important associations between scientific papers and patented inventions through a set of statistical measures introduced by our experts from the field of the Science of Science. A series of visualization views are then used to present these associations in the data context. In particular, we introduce the Interplay Graph to visualize patterns and insights derived from the data, helping users effectively navigate citation relationships between papers and patents. This visualization thereby helps them identify the origins of technical inventions and the impact of scientific research. We evaluate the system through two case studies with experts followed by expert interviews. We further engage a premier research institution to test-run the system, helping its institution leaders to extract new insights for innovation.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, December 2022

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/achieves/00_Abstract/00_Abstract_v1_20230312.tex <==
How science is consumed by the public domain (\eg, technology and public policy) has become a significant research question for understanding the broad impact of science. 
As one of these downstream fields, the interplay between science and technology has attracted the attention of various stakeholders (\eg, research institutions, companies, and science of science (SciSci) researchers). 
Understanding this interplay and identifying unrealized inventors and innovations can facilitate policy-making, knowledge transfer, and further drive innovation and economic growth in researchers' local communities and beyond. 
Recently, with the availability of well-structured science and technology-related data (\eg, papers, patents, and paper-patent citations), new avenues have been opened up for studying this interplay and gaining new insights. 
However, conventional statistical approaches fall short in addressing this problem adequately, given larger and multi-source datasets with complex network and temporal structures. 
We propose \systemname, an interactive visualization system for research institutions and SciSci researchers to \wyf{explore the interplay between science and technology and identify potential innovations, inventors, and technology partners intuitively and effectively}. 
We first propose a set of measures with our experts to characterize such interplay and applied a prediction model to uncover unrealized innovations that might lead to future technologies. 
We then developed an interactive visual analytics system to understand the interplay intuitively and interactively. 
An intuitive \interplayview is designed to reveal the interplay between science and technology in a scalable manner. 
We use \wyf{a quantitative performance evaluation}, two case studies, and an expert interview to demonstrate the effectiveness and usability of \systemname. 

==> sections/achieves/00_Abstract/00_Abstract_v2_20230313.tex <==
% Prof. Cao重写的版本
\abstract{
Scientific research has always been an important driving force in human development. However, for a long time, it has not been clear how science actually influences the development of technology. Answering this question will facilitate the development of more rational scientific research plans and further promote the rational usage of existing research results. With the increasing availability of papers, patents, and other relevant data that document human research activities, there is an opportunity to explore the above issue in greater depth. Existing statistic-based analysis approaches are difficult to present the complex correlation between papers and patents, thus failing to reveal the intrinsic connections between scientific research and technological innovation. To address this issue, we introduce \systemname, an interactive visual analysis system for researchers to explore the interplay between science and technology and identify critical innovations, inventors, and potential collaborators. The system first identifies important associations between research (papers) and technology (patents) through a set of statistical measures introduced by our experts from the field of science of science (SciSci). A series of interactive visualization views are then used to present these associations in the data context. In particular, we introduced \interplayview to visualize large-scale data associations and to clearly present the citations between patents and papers, thus helping users to identify the sources of technical inventions as well as the impact of scientific research. We evaluate the system through case studies with expert users followed by domain expert interviews. 


% How science is consumed by the public domain (\eg, technology and public policy) has become a significant research question for understanding the broad impact of science. 
% As one of these downstream fields, the interplay between science and technology has attracted the attention of various stakeholders (\eg, research institutions, companies, and science of science (SciSci) researchers). 
% Understanding this interplay and identifying unrealized inventors and innovations can facilitate policy-making, knowledge transfer, and further drive innovation and economic growth in researchers' local communities and beyond. 
% Recently, with the availability of well-structured science and technology-related data (\eg, papers, patents, and paper-patent citations), new avenues have been opened up for studying this interplay and gaining new insights. 
% However, conventional statistical approaches fall short in addressing this problem adequately, given larger and multi-source datasets with complex network and temporal structures. 
% We propose \systemname, an interactive visualization system for research institutions and SciSci researchers to \wyf{explore the interplay between science and technology and identify potential innovations, inventors, and technology partners intuitively and effectively}. 
% We first propose a set of measures with our experts to characterize such interplay and applied a prediction model to uncover unrealized innovations that might lead to future technologies. 
% We then developed an interactive visual analytics system to understand the interplay intuitively and interactively. 
% An intuitive \interplayview is designed to reveal the interplay between science and technology in a scalable manner. 
% We use \wyf{a quantitative performance evaluation}, two case studies, and an expert interview to demonstrate the effectiveness and usability of \systemname. 
} 



==> sections/achieves/00_Abstract/00_Abstract_v3_20230315.tex <==
\abstract{
Scientific research has long served as an important driving force in human development. 
However, for a long time, it has not been clear how science actually influences the development of technology. 
Answering this question can lead to more informed research plans and optimize the utilization of existing research findings. 
% Answering this question will facilitate the development of more rational scientific research plans and further promote the rational usage of existing research results. 
With the increasing availability of papers, patents, and other relevant data that document human research activities, opportunities arise to explore the above issue in greater depth. 
Existing statistic-based analysis approaches are difficult to present the complex relationships between papers and patents, thus hindering the revelation of intrinsic links between scientific research and technological innovation. 
% Existing statistic-based analysis approaches are difficult to present the complex correlation between papers and patents, thus failing to reveal the intrinsic connections between scientific research and technological innovation. 
To address this issue, we introduce \systemname, an interactive visual analysis system for research institutions and SciSci researchers to explore the interplay between science and technology and identify critical innovations, inventors, and potential collaborators. 
The system first identifies important associations between science (papers) and technology (patents) through a set of statistical measures introduced by our experts from the field of science of science (SciSci). 
A series of interactive visualization views are then used to present these associations in the data context. 
In particular, we introduced \interplayview to visualize large-scale data associations and to clearly present the citations between patents and papers, thus helping users to \wyf{identify the sources of technical inventions} as well as the impact of scientific research. 
We evaluate the system through two case studies with expert users followed by domain expert interviews. 
} 



==> sections/achieves/00_Abstract/00_Abstract_v4_20230319.tex <==
% Prof. Cao's Refinement
\abstract{
Scientific research has long served as an important driving force in human development. 
However, for a long time, it has not been clear how science actually influences the development of technology. 
Answering this question can lead to more rational research plans and promote the utilization of existing research findings. 
% Answering this question will facilitate the development of more rational scientific research plans and further promote the rational usage of existing research results. 
With the increasing availability of papers, patents, and other relevant data that document human research activities, opportunities arise to explore the above issue in greater depth. 
Existing statistic-based analysis approaches are difficult to present the complex relationships between papers and patents, thus hindering the revelation of intrinsic links between scientific research and technological innovation. 
% Existing statistic-based analysis approaches are difficult to present the complex correlation between papers and patents, thus failing to reveal the intrinsic connections between scientific research and technological innovation. 
To address this issue, we introduce \systemname, an interactive visual analysis system for research institutions and SciSci researchers to explore the interplay between science and technology and identify critical innovations, inventors, and potential collaborators. 
The system first identifies important associations between science (papers) and technology (patents) through a set of statistical measures introduced by our experts from the field of science of science (SciSci). 
A series of interactive visualization views are then used to present these associations in the data context. 
In particular, we introduced \interplayview to visualize large-scale data associations and to clearly present the citations between papers and patents, thus helping users to \wyf{identify the sources of technical inventions} as well as the impact of scientific research. 
We evaluate the system through two case studies with expert users followed by domain expert interviews. 


% How science is consumed by the public domain (\eg, technology and public policy) has become a significant research question for understanding the broad impact of science. 
% As one of these downstream fields, the interplay between science and technology has attracted the attention of various stakeholders (\eg, research institutions, companies, and science of science (SciSci) researchers). 
% Understanding this interplay and identifying unrealized inventors and innovations can facilitate policy-making, knowledge transfer, and further drive innovation and economic growth in researchers' local communities and beyond. 
% Recently, with the availability of well-structured science and technology-related data (\eg, papers, patents, and paper-patent citations), new avenues have been opened up for studying this interplay and gaining new insights. 
% However, conventional statistical approaches fall short in addressing this problem adequately, given larger and multi-source datasets with complex network and temporal structures. 
% We propose \systemname, an interactive visualization system for research institutions and SciSci researchers to \wyf{explore the interplay between science and technology and identify potential innovations, inventors, and technology partners intuitively and effectively}. 
% We first propose a set of measures with our experts to characterize such interplay and applied a prediction model to uncover unrealized innovations that might lead to future technologies. 
% We then developed an interactive visual analytics system to understand the interplay intuitively and interactively. 
% An intuitive \interplayview is designed to reveal the interplay between science and technology in a scalable manner. 
% We use \wyf{a quantitative performance evaluation}, two case studies, and an expert interview to demonstrate the effectiveness and usability of \systemname. 
} 



==> sections/achieves/01_Introduction/01_Introduction_v1_20230104.tex <==
% v1: 20230104 
\firstsection{Introduction}
\label{sec:01_introduction}
\maketitle 

How science is consumed outside of science (e.g., technology and public policy) has become an increasingly important topic to learn the broad impact of science~\cite{yin2022public, kostoff1997handbook}. 
As one of these downstream fields, the interplay between science and technology has attracted the attention of various stakeholders in academia and industry~\cite{ahmadpoor2017dual}. 
Research institutions such as universities aim to facilitate knowledge transfers from science produced by faculties to marketplace applications. 
Companies are interested in horizon scan~\cite{amanatidou2012concepts} and capture the cutting edge in science, which is potentially helpful to develop new products. 
Researchers in Science of Science (SciSci, ~\cite{fortunato2018science, wang2021science}) want to have a deeper understanding of such interplay in terms of long-term evolution. 
% between scientific and technological progress 

Recently, the growing availability of well-documented technological data (\eg, \textit{PatentsView}~\cite{patentsview} and private invention data at research institutions~\cite{liang2022systematic}) has shed new light on this topic, breaking through the shackles of analyzing data within science (\eg, \wyf{paper citation networks~\cite{henry2007nodetrix, dork2012pivotpaths} and topics~\cite{choo2013utopian, dou2013hierarchicaltopics}}). 
However, most work in social science operationalizes science-technology interplay into paper-patent citations and applies descriptive analysis with statistical approaches~\cite{ahmadpoor2017dual, yin2022public, liang2022systematic}. 
They can not provide a comprehensive view of the interplay between science and technology and are ill-suited for interactive exploration for different stakeholders. 
In addition, most of them stay in revealing the history while not taking a further step to suggest the future, which is essential to facilitate knowledge transfers. 
Visual analytics is thus an effective and intuitive approach to address these analytical demands. 
\wyf{Existing studies in the visualization community focus on either paper~\cite{narechania2021vitality, li2019galex} or patent~\cite{kutz2004examining, koch2010iterative, ankam2012exploring} visualization}. 
Hardly have they studied this interesting linkage, let alone analyzed resultant complicated problems with more complex data. 

However, designing such a system still faces three challenges. 
% 1. characterize the problem domain & new measures for different entities 
First, quantifying and evaluating different entities (\eg, researchers, papers, and patents) in terms of science usage in technology is difficult. 
In addition to measuring papers and patents, extracting information to reveal the interplay between papers and patents is more essential and difficult, given the heterogeneous citation network among the two entities. 
% 2. visualization challenge: 
% multi-entities for multi-variate, 
% network, 
% temporal, 
% and scalability to handle different amounts of data. -> hierarchical, 
Second, visually presenting this interplay is challenging. 
Such data are quite complex, with networks, multi-dimensions, and hierarchical structures of different entities. 
% Such data is with a complex structure which is with heterogeneous networks and multiple dimensions for different entities. 
Moreover, revealing the interplay from a temporal aspect aggravates the difficulty. 
Scalability is also a nonnegligible problem when analyzing such interplay from different levels of detail (LOD), such as the researcher, institution, and whole science levels. 
% 3. analytical challenge (prediction)
Third, providing recommendations to facilitate transferring from science to technology is non-trivial. 
Recommending individual papers and paper fields with high potential to be used in technology in the future requires capturing potential features and considering the temporal perspective. 

To address these challenges, we first characterize the problem domain and extract a list of measures with social science experts. 
Then we propose a new framework to recommend science papers and fields with high potential to be used in technology in the future. 
Based on historical data and recommendation results, we develop an interactive visualization system with multiple views to support analyzing the interplay between science and technology \wyf{from a temporal perspective}. 
Specifically, a \matrixview is designed to show the linkage between science and technology in a scalable manner. 
A \featureglyph reveals the multi-variate summary and comparison of a group of papers \wyf{with different variations}. % 目前有2-3种变体，refine based on效果  
The contributions are listed as follows: 

The contributions of this paper are listed as follows. 
\begin{compactitem}
    \item We characterize the problem domain of visual analytics of science and innovation in terms of knowledge transfers from science to technology.  
    \item We provide an analytical framework to analyze the science-technology interplay from understanding to the recommendation, including scientific measures and a recommendation algorithm. 
    \item We present \systemname, a visual analytics system for different users to explore the interplay between science and technology using intuitive interactions and scalable visualization. 
    \item We use three case studies, an expert interview, and \wyf{a quantitative study of the framework} to demonstrate the effectiveness and usability of \systemname. 
\end{compactitem}

% By incorporating historical and temporal facts, 



% The study of scientific and technological progress

% in understanding the broad impact of science. 

% What is the broad impact of science is an interesting question that attracts stakeholders from different . 


==> sections/achieves/01_Introduction/01_Introduction_v1_20230313.tex <==
% v2: 20230313
\firstsection{Introduction}
\label{sec:01_introduction}
\maketitle 

Understanding how science impacts sectors beyond academia, such as technology and public policy, has become an increasingly significant area of study to learn the broad impact of science~\cite{yin2022public, kostoff1997handbook}. 
Among these downstream fields, the interplay between science and technology has attracted various stakeholders to gain perspective on the use of scientific research in intellectual property~\cite{ahmadpoor2017dual}. 
% It has garnered attention from various stakeholders in academia and industry. 
Research institutions such as universities aim to facilitate knowledge transfer from scientific outputs produced by their faculties to practical applications in the marketplace.  
% ``Based on the early findings of this research, there are specific implications for the implementation of existing legislation or executive order. In particular, policymakers and university administrators should consider developing targeted policies or programs to encourage faculty members with high potential for technology transfer to engage more actively with their TTOs. These policies could include financial incentives, mentoring programs, and streamline administrative processes to make it easier for faculty to participate in technology transfer activities. By implementing these measures, universities can better harness the potential of their faculty to drive innovation and economic growth in their local communities and beyond.''
Companies seek to stay up-to-date with the latest scientific advancements (\ie, horizon scanning~\cite{amanatidou2012concepts}), as this knowledge can help drive the development of new products. 
Researchers in the Science of Science (SciSci~\cite{fortunato2018science, wang2021science}) field seek to gain a deeper understanding of such interplay \wyf{temporally} such as identifying hot areas in research and technology fields. 
% Researchers in Science of Science (SciSci, ~\cite{fortunato2018science, wang2021science}) want to have a deeper understanding of such interplay in terms of long-term evolution. 
% between scientific and technological progress 
% ``Use by investors (i.e. venture capital, private equity, angel investors, institutional investors, etc. ) to identify trends in certain disciplinary fields''
% ``It solves problems for universities as it provides a data-based method to identify potential innovations within the university and commercialization partnerships with the industry. This is important since interested corporations often fund academic research; also because patents often lead to revenues via licensing revenue and/or the establishment of startup companies.''  


In recent years, the availability of well-documented technological data, such as PatentsView~\cite{patentsview} and private invention data (\eg, invention disclosures) at research institutions~\cite{liang2022systematic}, has opened up new avenues for this research topic, 
breaking through the shackles of analyzing data within science (\eg, \wyf{paper topics~\cite{choo2013utopian, dou2013hierarchicaltopics} and citation networks~\cite{henry2007nodetrix, dork2012pivotpaths}}). 
However, most social science research in this area relies on descriptive and statistical approaches that operationalize science-technology interplay solely through paper-patent citations~\cite{ahmadpoor2017dual, yin2022public, liang2022systematic}. 
They fail to provide a comprehensive and systematic view of this problem and are ill-suited for interactive exploration. 
Moreover, they tend to focus on revealing historical insights while not taking a further step to suggest the future, which is essential to facilitate knowledge transfer. 
% 
Visual analytics is an effective and intuitive approach to solving these analytical demands. 
\wyf{Nevertheless, existing studies in the visualization community have primarily focused on either paper~\cite{narechania2021vitality, li2019galex} or patent~\cite{kutz2004examining, koch2010iterative, ankam2012exploring} visualization} separately, and rarely have they studied this interesting linkage. 
As a result, they are ill-equipped to analyze this complicated problem that arises when dealing with more complex data. 

Designing such a visual analytics system faces three challenges. 
% 1. characterize the problem domain & new measures for different entities 
First, quantifying and evaluating different entities (\eg, researchers, papers, and patents) in terms of science usage in technology is difficult. 
In addition to measuring papers and patents separately, extracting information to reveal the interplay between papers and patents is vital and difficult, given the complex citation network and multi-dimensional nature of entities. 
% 2. visualization challenge: 
% multi-entities for multi-variate, 
% network, 
% temporal, 
% and scalability to handle different amounts of data. -> hierarchical, 
Second, visually presenting this interplay poses a challenge due to the complexity of the data, which includes networks, multi-dimensions, and hierarchical structures of various entities. 
% Second, visually presenting this interplay is challenging. 
% Such data are quite complex, with networks, multi-dimensions, and hierarchical structures of different entities. 
% % Such data is with a complex structure which is with heterogeneous networks and multiple dimensions for different entities. 
Moreover, revealing the interplay from a temporal aspect aggravates the difficulty. 
Scalability is also a nonnegligible issue when analyzing such interplay from different levels of detail (LOD), such as the individual researcher, the institution, the research field, and the whole science levels. 
% 3. analytical challenge (prediction)
Third, providing recommendations for different entities to facilitate knowledge transfer from science to technology is non-trivial. 
A useful prediction model and intuitive visualization approach should be adopted to identify potential innovations and fields in science and uncover talents with high unrealized potential for commercialization. 
% , and find potential technology partners for future collaboration. 
% Recommending paper fields and individual papers with high potential to be used in technology in the future requires capturing potential features and considering the temporal perspective. 
% Recommending innovations and fields, inventors with high potential to be used in technology in the future requires capturing potential features and considering the temporal perspective. 

To tackle these challenges, we first characterize the problem domain and define a list of measures with our domain experts. 
We then apply a prediction model to recommend science papers and fields with high potential to be used in technology in the future, which further indicates a list of researchers whose works are with high potential for commercialization/ 
Based on historical and recommendation results, we develop an interactive visualization system with multiple views to analyze the interplay between science and technology \wyf{from different aspects}. 
Specifically, a \interplayview is designed to show the linkage between science and technology in a scalable manner. 
A \featureglyph reveals the multi-variate summary and comparison of a group of papers \wyf{with different variations}. % 目前有2-3种变体，refine based on效果  
The contributions are listed as follows: 

The contributions of this paper are listed as follows. 
\begin{compactitem}
    \item We characterize the problem domain of visual analytics of science and innovation \wyf{in terms of the interplay of science and technology}. 
    \item \wyf{We provide an analytical framework to analyze the science-technology interplay from understanding to the recommendation, including a set of scientific measures and a prediction algorithm.} 
    \item We introduce \systemname, a visual analytics system that allows different users to investigate the interplay between science and technology through intuitive interactions and scalable visualization. 
    \item We use \wyf{a quantitative performance study}, two case studies, and an expert interview to demonstrate the effectiveness and usability of \systemname. 
\end{compactitem}

% By incorporating historical and temporal facts, 



% The study of scientific and technological progress

% in understanding the broad impact of science. 

% What is the broad impact of science is an interesting question that attracts stakeholders from different . 


==> sections/achieves/03_Background/03_Background_0326.tex <==
\section{Background}
\label{sec:03_Background} 
In this section, we first formulate the problem domain with experts and introduce the data sources. 
Then we distill analytical tasks based on the problem domain. 
Finally, we provide a system overview. 

\subsection{Problem Formulation} 
\label{sec:03_Background_ProblemFormulation} 
Over the past ten months, we have worked closely with experts from multiple fields. 
% who are interested in the interactions between science and technology. 
Two experts are from the technology transfer office (TTO) of a university: 
\ea is a senior director of invention management who aims to help faculty convert their scientific output into patents. 
\eb is an analyst providing data-driven support. 
The other two experts are SciSci researchers. 
\ec is a professor who is well-established in this field. 
\ed is a postdoc and focuses on science and innovation. 
% Lastly, \ee is a preeminent economist and professor with expertise in innovation, specifically in analyzing the relationship between science and technology. 
\wyf{Our goal is to analyze the interactions between science and technology in terms of different entities (\eg, researchers and scientific and technological fields). 
In addition to historical insights, the experts also wanted suggestions to identify untapped innovation potentials for the future.} 
However, their current analytical methods are mainly statistical and ad-hoc, with no known systematic approach to the issue.
% Yet, the current analytical approach of our experts is statistical and ad-hoc. 
% To the best of their knowledge, no others have tried to solve this problem in a more systematic way. 
% ``this is an empty market space to leverage big data on science and innovation to build tools to help the technology transfer office in research institutions and companies to identify unrealized innovations and find hidden connections that might lead to partnerships.'' 
% ``Current solutions are mainly based on experts' knowledge in a manual way and thus lack a systematic and automatic way to solve this problem.'' -- patent disclosure 
Through discussions with our experts, we finally formulated three analytical goals. 
% three-step analytical workflow: 

\noindent \textbf{\tasktypeone (\tasktypeoneshort).} 
% 对应左边2个view
As understanding individuals is critical and highly related to policy-making to facilitate knowledge transfer,  
the first goal is to investigate researchers, particularly those with considerable unrealized commercialization potential.
% The first goal of our experts is thus to explore researchers. 
% They are particularly interested in those with high unrealized potential for commercialization. 
The experts also aim to assess the current state of innovation opportunities and possible inequality issues in patenting activities within research institutions.
% In addition, the status quo of innovation opportunities is also essential. 
% Researchers may experience inequality issues in patenting activity within a research institution. 
For example, 
\textit{are there any group of researchers that innovation managers pay less support to (\eg, females)?} 
\wyf{The current analysis is mostly based on experts' domain knowledge due to the lack of proper measures.} 
% \textit{``Whose research has already been transformed into technology by themselves? 
% Whose research has high commercialization potential? Are they themselves aware of it or not?'' } 
% method: at a given research institution whose research publications have been cited in another organization's patents 
% ``Our proposed methodology aims to uncover untapped potential for commercialization at research institutions by identifying faculty members with patentable works who have been producing research with translational impact but have not yet engaged significantly with the university technology transfer office (TTO). '' 
% ``To achieve this, we will develop measurements to gauge the potential of faculty members and evaluate their current engagement with TTO by leveraging public data on papers, patents, and the citation linkages between them, as well as private data including (i) faculty’s invention disclosures and outcomes on patent filing, granting, licensing, and startups from TTO. (ii) faculty roster with demographic data from HR.; (iii) faculty’s grant application data (both successful and failed attempts) and these grant applications’ outcomes from the sponsored research office from several top universities where active negotiations are underway for data transfers. A pilot study is currently underway at Northwestern University.''
% ``Based on the early findings of this research, there are specific implications for the implementation of existing legislation or executive order. In particular, policymakers and university administrators should consider developing targeted policies or programs to encourage faculty members with high potential for technology transfer to engage more actively with their TTOs. These policies could include financial incentives, mentoring programs, and streamline administrative processes to make it easier for faculty to participate in technology transfer activities. By implementing these measures, universities can better harness the potential of their faculty to drive innovation and economic growth in their local communities and beyond.''

\noindent \textbf{\tasktypetwo (\tasktypetwoshort).} 
% 对应mainview + 右边2个view 
Another goal of our experts is to learn the interactions between science and technology, either focusing on specific researchers or scientific fields. 
In addition to citation linkages, other information about science and technology is wanted to facilitate the interpretation of such interplay. 
% After locating an interesting group of researchers, 
% the experts aim to obtain further details about the \wyf{translational impact of their research~\cite{??}}, which can be captured by how their papers are cited in patents. 
Statistical approaches are commonly applied in the SciSci field to analyze paper-patent citations. 
However, they typically focus on a specific aspect of the problem and it is difficult to get a global view of such interactions from multiple levels of detail. 
% a back-and-forth analytical pipeline requires much analytical effort
% it cannot support multi-level analysis among different paper and patent fields. 
% Moreover, 
% given multiple aspects of interest (\eg, papers, patents, and paper-patent linkages), 
% Moreover, the result presentation is typically static charts, which are limited to a subset of science or technology fields and cannot provide an interactive and scalable view of such interplay from different LODs. 
Thus, this step aims to assist experts in exploring the connection between science and technology intuitively and effectively. 

% \noindent \textbf{\tasktypethree (\tasktypethreeshort).} 
% In addition to historical analysis, our experts also indicating 
% science fields with high potential to be patentable in the future are also highly demanded by experts. 


\noindent \textbf{\tasktypethree (\tasktypethreeshort).} 
% 对应所有含有prediction result的view (all views except 右上角)
% identify: (1) partners (2) papers that are patentable
% junior scholar进到NU，还没有historical data，有bias，
The conventional analysis of this problem is mostly based on observations of historical data. 
However, our experts also mentioned the importance of providing suggestions to make evidence-based decision-making. 
Thus, prediction and recommendation should be considered in this step to indicate the future. 
Different \wyf{entities} are required to be involved in this process. 
For example, 
\textit{what recently published papers or science fields have a high translational impact that could result in patents and technologies?} 
\textit{How to find potential partners and collaboration topics for research institutions to facilitate knowledge transfer?} 
% when patent may be forthcoming given the identification of papers that have characteristics that might lead to future patents
% ``It solves problems for universities as it provides a data-based method to identify potential innovations within the university and commercialization partnerships with the industry. This is important since interested corporations often fund academic research; also because patents often lead to revenues via licensing revenue and/or the establishment of startup companies.''
% ``Use by academic research institutions to identify potential research and/or commercialization partners'' 


% =============== Data Description ===============
\subsection{Data Description} 
\label{sec:03_Background_DataDescription} 
Analyzing the dual frontier of science and technology requires aggregating data from multiple sources, including large-scale datasets tracing scientific publications and patented inventions, and the complex interactions among them. 
We summarize data sources used in our work. 
\begin{compactitem}
    \item \textbf{Science Data} are from Microsoft Academic Graph (MAG)~\cite{sinha2015overview}, which records meta information about 271M papers, \eg, publication year, title, doi, citation linkages among papers, and authors and their affiliations, across all scientific fields.
    \item \textbf{Technology Data} are from PatentsView~\cite{patentsview}, which records over 7.9M patent records from the United States Patent and Trademark Office (USPTO~\cite{uspto}). 
    We only use a subset of attributes including patent id and title, application year, assignee name (\ie, the owner of the patent), and cooperative patent classification (CPC, \ie, the category of the patent~\cite{cpcscheme}). 
    % (\ie, the entity to whom the patent rights have been transferred or assigned. In other words, the assignee is the owner of the patent.)
    In some cases, 
    % (\eg, Case 1 in Section~\ref{sec:06_Evaluation}), 
    private data such as faculty's invention disclosures and their patents collected by research institutions will also be used. 
    \item \textbf{Science-Technology Linkage Data} from Reliance on Science~\cite{marx2020reliance, marx2022reliance} are an important source in this work, which provides 40M citation linkages from patents to papers. 
    \item \textbf{Researcher Data} include demographic information (\eg, gender, rank, and affiliation), which are collected by research institutions or inferred by algorithms~\cite{karimi2016inferring}). 
    The linkage between researchers and papers is either from the public dataset (\eg, MAG) or the private dataset (\eg, university private records). 
    % \item \textbf{Faculty Data}. 
    % We collected private demographic information (such as gender and academic rank) and private data on invention disclosures for faculty from the universities that we partnered with. 
    % 
    % As researchers are one of the essential entities in our scenario, we also integrate multi-dimensional data from researchers, including
    % collected by research institutions or inferred by algorithms~\cite{karimi2016inferring}) and calculated SciSci metrics (\eg, paper citations).
    % The linkage between researchers and papers is either from the public dataset (\eg, MAG) or private dataset (\eg, \wyf{university private records}). 
    % \item \textbf{\wyf{Organization Data}}. 
    % \wyf{Organization: Global Research Identifier Database (GRID). } 
\end{compactitem}

\subsection{Analytical Tasks} 
\label{sec:03_Background_AnalyticalTasks} 
After figuring out the above goals, we continue to distill and refine analytical tasks iteratively with our expert following the nested model of visualization design~\cite{munzner2009nested}. 
The process includes a literature review with SciSci experts, regular weekly interviews and brainstorming with all experts and other visualization researchers. 
We finally formed the following tasks as follows.  
% ``It solves problems for universities as it provides a data-based method to identify potential innovations within the university and commercialization partnerships with the industry. This is important since interested corporations often fund academic research; also because patents often lead to revenues via licensing revenue and/or the establishment of startup companies.''  

\vspace{1mm}
\noindent \textbf{\tasktypeone (\tasktypeoneshort).} \\
% Scatterplot View
\noindent \textbf{\tasktypeoneshort1: Generate an overview of researchers.} 
 % in terms of \wyf{science and technology performance}.
Given a list of researchers (\eg, university faculties or researchers in a science field), such an overview should reveal different groups in terms of their work in science and technology and guide experts to select interested groups in the following analysis. 
Thus, the experts requested to distill suitable metrics for each researcher and use intuitive visualization to show the overview. 
% method: scisci measures are required

% Researcher Statistics View 
\noindent \textbf{\tasktypeoneshort2: Portrait the talents.} 
After choosing a group of interest, two aspects are required by our experts to portray these researchers to understand their characteristics. 
First, demographic information (\eg, gender and job rank) is useful to learn diversity, equity, and inclusion (\ie, DEI) in terms of innovation opportunities and facilitate equality. 
% potential inequality phenomena and facilitate equality. 
% For example, \textit{are female researchers with fewer inventions in this institution?} 
% If yes, is it because the institution has paid less attention to them to help them transfer research knowledge?'' 
Second, the experts wanted suitable metrics to summarize their scientific and technological outputs. 
% the experts also wanted suitable measures to summarize the scientific and technological performance of these researchers. 
Moreover, the experts also mentioned the necessity of tracing individual researchers to find potential inventors. % statistics -> paper card 
% ``- Identify innovation opportunity at the demographic level at Northwestern:
%     - Identify and support female inventors.
%     - Support inventive activities from tenure-track faculty.
%   - Identify faculty with high unrealized potential for commercialization''

\vspace{1mm}
\noindent \textbf{\tasktypetwo (\tasktypetwoshort).} \\ 
\noindent \textbf{\tasktypetwoshort1: Inspect the interaction between science and technology.} 
% 1. multi-level, 不同粒度
Given large-scale data about papers and patents, our experts expected an intuitive and scalable visual representation to explore this linkage from different levels of detail (LOD), such as course-grained research fields and fine-grained one researcher's works. 
They also wanted the visualization to be easy to interact with to filter data of interest. 
% 2. glyph + multi-attribute + Y-axis设计的理由
In addition, they are particularly interested in what characteristics are associated with their use in technology. 
% They wanted to locate papers significantly used by patents and find why they are more likely to be transformed into technology by comparing them with other papers. 

\noindent \textbf{\tasktypetwoshort2: \wyf{Reveal evolving trends in science and technology fields.}} 
% \noindent \textbf{\tasktypetwoshort2: \wyf{Identify hot areas in science and technology fields.}} 
Most current analysis stands on the present and aggregate historical interplay altogether. 
However, our experts are also interested in studying the evolution of the dual frontiers between science and technology. 
Temporal trends are of critical importance not only for comprehending the fluctuations of fields but also for identifying burgeoning domains in science and technology. 
Such insights can be utilized to facilitate the transfer of knowledge in the present. 
% Such temporal trends are not only essential to learn the rise and fall of fields but also can help identify hot areas in science and technology to facilitate knowledge transferring at present. 

\noindent \textbf{\tasktypetwoshort3: Reason the interaction with contextual information.} 
In addition to showing the citation linkages, other data aspects should also be considered to understand the holistic impact of scientific research. 
For patents, assignees and patent topics are essential for experts to identify commercialization and partnership potential. 
For papers, overall distributions of different metrics and detailed individual papers are required by experts to comprehend \wyf{science and technology performance}. 

\vspace{1mm}
\noindent \textbf{\tasktypethree (\tasktypethreeshort).} \\
\noindent \textbf{\tasktypethreeshort1: Identify untapped innovation potentials.} 
In addition to understanding the linkages between science and technology in the past, our experts also want suggestions to uncover untapped innovation potentials in researchers, scientific fields, and research topics. 
% suggesting potential partners from the technology aspect, our experts also want to find recent science papers with high potential to be patentable in the future. 
This critical step can significantly facilitate knowledge transfer for the latest scientific publications. 
Thus, a rational prediction model and intuitive visualization should be incorporated to reveal the future direction. 
% ``help investors and/or funders understand when patent may be forthcoming given the identification of papers that have characteristics that might lead to future patents'' 
% ``We developed a systematic framework for identifying research faculty in the United States with high untapped commercialization potential.''

% \wyf{
% \noindent \textbf{\tasktypeoneshort1: Identify Commercialization and Partnership Potential.} 
% Bridging research institutions and companies consuming their knowledge is essential since it can help them make previously invisible connections to land scientific knowledge. 
% Our experts are eager to find potential partners from companies and other \wyf{technical organizations} through intuitive visualization.  
% In addition, such visualization should also support revealing the potential collaboration topics in the technology in a more fine-grained way. 
% method: by identifying those organizations that have cited a research institute's publications in their patents. 3) Aggregate the companies which are most frequently citing a given research institution's research publications 
% } 

% \wyf{
% \noindent \textbf{\tasktypeoneshort2: Identify unrealized innovations that might lead to future patents.} 
% % Paper Inspection View + prediction model 
% In addition to suggesting potential partners from the technology aspect, our experts also want to find recent science papers with high potential to be patentable in the future. 
% This critical step can significantly facilitate knowledge transfer for the latest scientific publications. 
% Thus, a prediction model and intuitive visualization should be incorporated to reveal the future direction. 
% % ``help investors and/or funders understand when patent may be forthcoming given the identification of papers that have characteristics that might lead to future patents'' 
% % ``We developed a systematic framework for identifying research faculty in the United States with high untapped commercialization potential.''
% }

\subsection{System Overview} 
\label{sec:03_Background_SystemOverview} 
\systemname is a web-based application consisting of three modules (Fig.~\ref{fig:system-overview}), namely, a data storage module, a data analysis module, and a data visualization module. 
The data storage module preprocesses multiple data sources and stores them in a database. 
The data analysis module conducts a set of measures about science and technology on different entities (\eg, papers, patents, and researchers) and uses a prediction model to recommend papers with high potential to be patentable. 
The two module forms the backend of the system. 
% The two module forms the backend of the system and is implemented by MongoDB~\cite{mongodb} and Python~\cite{python}. 
Both historical and prediction data are then fed into the data visualization module to present intuitive and interactive data insights. 
% It is implemented by React.js~\cite{react} and D3.js~\cite{bostock2011d3}. 


\begin{figure} [!htb]
 \centering 
%  \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figures/system-overview-20230325.png}
%  \vspace{-0.5cm}
 \caption{System overview. \systemname consists of a data storage module, a data analysis module, and a data visualization module.} 
%  \vspace{-0.4cm}
 \label{fig:system-overview}
\end{figure}

==> sections/achieves/04_DataAnalysis/04_DataAnalysis_20230326.tex <==
% yifan's initial version

\section{Data Analysis}
\label{sec:04_DataAnalysis} 

\subsection{Data Preprocessing} 
\label{sec:04_DataAnalysis_DataPreprocessing}  
% 比如patent是univeristy还是company性质的也是我们处理过后得到的 
% paper topic 3层写在这里好了：L0/L1/L2
For our study, we are specifically examining papers published between 2001 and 2020. Every paper in MAG is linked to several fields of study, which have been classified into a hierarchical taxonomy consisting of several levels. For our study, we have retained the top four levels, ranging from L0 to L3, where L0 denotes broad fields such as computer science and biology, while L2, L3, and L4 correspond to increasingly specific subfields. In PatentsView, each patent is linked to multiple CPC categories, which are organized into a hierarchical taxonomy with several levels. For the purposes of our study, we have limited our analysis to the top three levels, consisting of CPC section, CPC subsection, and CPC group. The broadest level, CPC section, encompasses broad technical fields, such as Section A: "Human Necessities". The CPC subsection and group levels provide increasingly specific subcategories within each section.

For case 1 in Section~\ref{sec:06_Evaluation_CaseStudy_Case1_NU}, we focus on $461$ faculty who have at least one paper that has been cited by a patent and their 37K papers which enables us focusing on researchers whose papers have impact on patents.

To identify potential innovators in case 2 in Section~\ref{sec:06_Evaluation_CaseStudy_Case2_VIS}, we extracted papers from six top journals and fourteen leading conferences in the fields of VIS and HCI. We then narrowed our focus to authors who had published at least ten papers in these venues. Next, we examined all papers published by these authors and retained only those who had at least five papers cited by patents. Our final dataset included $2,016$ VIS and HCI researchers and a total of 129K papers authored by them, meeting the aforementioned criteria.

\subsection{SciSci Metric based on Historical Facts} 
\label{sec:04_DataAnalysis_SciSciMeasure} 
\subsubsection{Paper metric} 
\wyf{We obtained a list of paper metrics with our domain experts from the SciSci field, which are listed below. }
% \wyf{We leveraged several SciSci metrics provided from \YQ{SciSciNet} which built on MAG and other related open-source data sets.} 
\begin{compactitem}
    \item \variable{team size}: the number of authors of the focal paper. 
    \item \variable{institution count}: the number of institutions associated with the focal paper. 
    \item \variable{NSF count} and \variable{NIH count}: the number of NSF or NIH grants supporting the focal paper. 
    % \item \variable{NIH count}: the number of NIH grants supporting the focal paper. 
    \item \variable{5-year science citation}: the number of times a focal paper is cited by other papers within a 5-year period of its publication. 
    \item \variable{disruption}: the degree to which papers citing the focal paper tend not to cite the references of the focal paper~\cite{wu2019large}.
    \begin{equation}
        D = \frac{n_i - n_j}{n_i + n_j + n_k}
    \end{equation}
    \noindent where $n_i$ represents the number of subsequent papers that only cite the focal paper, $n_j$ represents the number of subsequent papers that cite both the focal paper and its references, and $n_k$ represents the number of subsequent papers that cite the references of the focal paper only.
    \item \variable{novelty}: The 10th percentile z-score of a paper's journal pair references captures how much the focal paper's combination of existing knowledge deviates from the norm among all journal pairs. The z-score of a journal pair is computed by comparing its observed frequency to the expected frequency in randomized citation graphs, as proposed by Uzzi et al. in their work on atypical combinations of knowledge~\cite{uzzi2013atypical}.
    \item \variable{5-year patent citation}: the number of patent citations received by a paper within 5 years of its publication. It is the time difference between the application year of citing patent and the publication year of the cited paper. 
\end{compactitem} 
% Additionally, we computed the number of patent citations received by a paper within 5 years of its publication. 
% This was determined by examining the difference between the filing year of citing patent and the publication year of the cited paper.

\subsubsection{Researcher metric}
% 要说一下measure是从paper集成到人的。左下是人的measure，右下是paper的
Using metrics associated with a researcher's papers, we computed several related metrics to describe their performance in science and impact on patents, including (1) number of papers; (2) average 5-year science citations; (3) number of papers cited by patents; (4) number of patents citing the researcher's papers; (5) number of patent citations. In addition, we used an institution's internal data to count the (6) researcher's number of invention disclosures and (7) number of granted patents.  

\subsection{SciSci Metric based on Prediction Models}
\label{sec:04_DataAnalysis_PredictionModel} 
% Yifan: please add here
% (1) please add gnn/other related work reference here. 
% (2) justification required: 
% 1. input为什么是text + graph? -> 单独prediction的效果都没有合起来好
% 2. cpc group为什么是top 50? justify 50这个数值
% p-index感觉应该写在prediction model后面
\subsubsection{Paper metric}
To evaluate the potential translational impact of recently published papers on technology, relying solely on whether they receive patent citations is not adequate as they may not have had sufficient time to accrue citations. For example, for papers published within the past year, it is crucial to predict their translational potential, as researchers can still patent their work within one year of publication. After this period, the paper becomes fully public knowledge and cannot be patented or further commercialized, even if it later turns out to have high commercial value.. In such scenarios, a machine learning model needs to be constructed to predict the probability of receiving patent citations within $t$ years of publication. Here, we have set $t=5$ without loss of generality.

To exemplify the prediction model, we will use the case 1 as a running example. We investigated whether each paper published between 2001 and 2015 was cited by a patent from each of the top $50$ patent CPC groups that cited Northwestern's papers, within 5 years of its publication year. We denote the set of $50$ patent CPC groups as $\mathbb{G}$. The top $50$ CPC groups account for the vast majority of patents (over 95\%) citing Northwestern's papers. 

To construct the prediction model, we employ both the semantic content of papers and the structural relationships between them. First, we utilize SPECTER~\cite{specter_cohan_2020} to embed the paper's title into a high-dimensional feature vector, which encodes its semantic content. Second, we create a citation graph, where each node represents a paper, and an undirected link connects two papers if one paper cites the other. The two different data sources we use, semantic embedding of paper titles and citation relationships between papers, can offer unique and valuable information for predictions~\cite{qian2021quantifying,qian2021geometric}. The semantic embedding of a paper's title can provide insights into the topics covered in the paper, which can indicate the likelihood of it being cited in a patent and in which patent category. On the other hand, the citation relationships between papers can also provide useful information as a paper citing other papers that have already been cited in patents may indicate that the focal paper may also be cited in patents. Since both sources of information can contribute to better prediction performance, our aim is to leverage a machine learning model that can effectively combine both sources of data as inputs and be trained in an end-to-end manner without relying on sophisticated feature engineering with domain knowledge. To this end, Graph Neural Networks (GNNs) are a natural choice for achieving this goal~\cite{bronstein2017geometric}, as they can effectively integrate both the features of each paper and the citation graph structure to learn meaningful representations of the papers. GNNs have shown great success in various tasks, including classifications, and are thus a promising approach for our prediction model. Specifically, we utilize Graph Convolutional Networks (GCNs)~\cite{kipf2017semi}, which are the canonical GNN models that have played a significant role in popularizing the GNN family of models.

Following the approach of the GCN paper~\cite{kipf2017semi}, we formulated our prediction tasks as a semi-supervised learning problem. As of the end of 2020, which is the most recent year in our system, we constructed the citation network between \YQ{Northwestern papers} published between 2001-2020, described by an adjacency matrix $A \in \mathbb{R}^{N \times N}$. Each paper is associated with a F-dimensional vector embedded from the SPECTER based on its title, which is arranged as a row of the feature matrix $X \in \mathbb{R}^{N \times F}$. For $N_{s}$ papers published between 2001-2015, for one patent CPC group $g$, we associated the paper with one of the $2$ classes, which is encoded into a 0-1 membership matrix $Y \in \mathbb{R}^{N_{s} \times 2}$ to indicate whether the paper is cited by patents from the CPC group $g$.

Our study applies the two-layer GCN proposed in~\cite{kipf2017semi}. Given the feature matrix X and the adjacency matrix A, the propagation rule is given by:

\begin{equation}
Z=f(X, A)=\mathrm{softmax}\left(\widehat{A} \mathrm{ReLU}\left(\widehat{A} X W^0\right) W^1\right)
\end{equation}

\noindent  where $W^{0}$ and $W^{1}$ are the weights connecting the layers of the GCN. The graph is encoded in
$\widehat{A}=\widetilde{D}^{-1/2}(A + I_{N})\widetilde{D}^{-1/2}$, where $I_{N}$ is the identity matrix, and $\widetilde{D}$ is a diagonal matrix with $\widetilde{D}_{ii} = 1 + \sum_{j}A_{ij}$. The softmax output $Z \in \mathbb{R}^{N \times 2}$ contains two probabilities for each paper, indicating the likelihood of the paper being cited by patents or not. The $\mathrm{softmax}$ and $\mathrm{ReLU}$ are threshold activation functions:

\begin{align}
\mathrm{ReLU}(x)_{i}=\max(x_{i},0)  \\
\mathrm{softmax}(x)_{i} = \frac{\exp(x_{i})}{\sum_{j} \exp(x_{j})}
\end{align}

\noindent where $x$ is a vector. For semi-supervised classification, we then evaluate the cross-entropy error over all the papers in the training set:

\begin{equation}
        \mathcal{L} = -\displaystyle\sum_{l\in \mathbb{N}_{T}}\displaystyle\sum_{c=1}^{2} Y_{lc} \, \ln{Z_{lc}},
    \label{eq:cross_entropy_error}
\end{equation}

\noindent where $\mathbb{N}_{T}$ is the set of papers in the training set. The weights of the neural network ($W^{0}$ and $W^{1}$) are trained using gradient descent to minimize the loss~$\mathcal{L}$. 

We split the papers published between 2001-2014 into a training set (70\%) and a validation set (30\%), and use papers published in 2015 as the test set. For each paper published between $2016$-$2020$, we predict its likelihood of being cited by patents in CPC group $g$. We use the PyTorch Geometric implementation of GCN~\cite{Fey/Lenssen/2019} and follow the experimental setup in~\cite{kipf2017semi}. Our GCN model consists of two layers with $200$ epochs of training iterations, a learning rate of $0.01$, a dropout rate of $0.5$, and $16$ hidden units, which are model default parameters. Due to the class imbalance between papers that receive patent citations and those that do not, we evaluate the performance of our model using the AUC (Area Under the Curve) metric which is is a common evaluation metric for imbalanced binary classification problems. Our final model is chosen from the epoch that produces the highest AUC score on the validation set. To assess the performance of the model, we report its AUC on the test set.

To determine the likelihood of a paper $k$ published between $2016$-$2020$ being cited by patents in the CPC group $g$ within $5$ years of publication, we make use of the predicted probabilities in the softmax output matrix $Z$ obtained from the final model. In order to assess its relative importance within Northwestern, we convert its probability to a percentile by determining where it falls within all Northwestern papers published between $2016$-$2020$, denoted as $\text{Patentability}_k^g$, which is a scalar ranging from 0 to 100.

We iterate the above process on all the CPC groups in $\mathbb{G}$. For a paper $k$ published between $2016$-$2020$, to further summarize its overall patentability, we take the average $\text{Patentability}(k,g)$ across CPC groups $g$ in $\mathbb{G}$ as $\text{Patentability}_k$. Similarly, we also repeat our analysis on case 2.

\subsubsection{Researcher metric}
We examined the predicted $\text{Patentability}_k$ of a researcher's papers published from 2016 to 2020, and computed the average as their P-index, which summarizes the predicted translational impact on patents of their research.


==> sections/achieves/04_DataAnalysis/04_DataAnalysis_20230327_after_yifang.tex <==
\section{Data Analysis}
\label{sec:04_DataAnalysis} 
In this section, we introduce our data analysis approach, including preprocessing, SciSci metric calculation, and prediction model. 

\subsection{Data Preprocessing} 
\label{sec:04_DataAnalysis_DataPreprocessing}  
After collecting multiple sources in Section~\ref{sec:03_Background_DataDescription}, we preprocess them to fit our scenario. 
First, we focused on the paper-patent linkage between 2001 and 2020 as an example to demonstrate our idea. 
Thus we specifically examined papers published between 2001 and 2020. 
Second, since we were particularly interested in researchers whose works have the potential to be cited by patents, we filtered to get researchers who have at least one paper that has been cited by a patent. 
Third, for patent assignees, we used keyword matching to semi-automatically classify patents into three categories: university assignees, company assignees, and others. 
All the results were fed into the following analysis steps. 
% Every paper in MAG is linked to several fields of study, which have been classified into a hierarchical taxonomy with multiple levels. 
% For our study, we have retained the top four levels, ranging from L0 to L3, where L0 denotes broad fields such as computer science and biology, while L2, L3, and L4 correspond to increasingly specific subfields. 
% In PatentsView, each patent is linked to multiple CPC categories, which are organized into a hierarchical taxonomy with several levels. 
% For the purposes of our study, we have limited our analysis to the top three levels, consisting of CPC section, CPC subsection, and CPC group. 
% The broadest level, CPC section, encompasses broad technical fields, such as Section A: "Human Necessities". 
% The CPC subsection and group levels provide increasingly specific subcategories within each section. 
% In this study, we are specifically examining papers published between 2001 and 2020. 


\subsection{SciSci Metric based on Historical Facts} 
\label{sec:04_DataAnalysis_SciSciMeasure} 
\subsubsection{Paper Metric} 
\wyf{We defined and obtained a list of metrics for each paper with experts from the SciSci field, which are highly related to our analytical problem. }
% \wyf{We leveraged several SciSci metrics provided from \YQ{SciSciNet} which built on MAG and other related open-source data sets.} 
\begin{compactitem}
    \item \textit{team size}: the number of authors of the focal paper. 
    \item \textit{institution count}: the number of institutions associated with the focal paper. 
    \item \textit{NSF count} and \textit{NIH count}: the number of NSF or NIH grants supporting the focal paper. 
    \item \textit{5-year science citation}: the number of citations a focal paper obtains within a 5-year period from its publication. 
    \item disruption: the degree to which papers citing the focal paper tend not to cite the references of the focal paper~\cite{wu2019large}.
    \begin{equation}
        D = \frac{n_i - n_j}{n_i + n_j + n_k}
    \end{equation}
    \noindent where $n_i$ represents the number of subsequent papers that only cite the focal paper, $n_j$ represents the number of subsequent papers that cite both the focal paper and its references, and $n_k$ represents the number of subsequent papers that cite the references of the focal paper only.
    \item \textit{novelty}: also known as the 10th percentile z-score of a paper's journal pair references, which captures how much the focal paper's combination of existing knowledge deviates from the norm among all journal pairs. 
    The z-score of a journal pair is computed by comparing its observed frequency to the expected frequency in randomized citation graphs~\cite{uzzi2013atypical}. 
    % , as proposed by Uzzi \etal in their work on atypical combinations of knowledge~\cite{uzzi2013atypical}.
    \item \textit{5-year patent citation}: the number of patent citations received by a paper within 5 years from its publication. 
    The time difference is defined by the duration between the application year of citing patent and the publication year of the cited paper. 
    % It is the time difference between the application year of citing patent and the publication year of the cited paper. 
\end{compactitem} 


\subsubsection{Researcher Metric}
Based on paper metrics, we aggregated a list of researcher metrics at the individual level to describe his/her performance in science and impact on patents, including \textit{number of papers}, \textit{average 5-year science citations}, \textit{number of papers cited by patents}, \textit{number of patents citing the researcher's papers}, \textit{number of patent citations}. 
In addition, we used an institution's internal data to count the \textit{researcher's number of invention disclosures} and \textit{number of granted patents}. 

\subsection{SciSci Metric based on the Prediction Model}
\label{sec:04_DataAnalysis_PredictionModel} 
In addition to metrics based on historical data, we also apply a prediction model to evaluate the potential translational impact of recently published papers on technology. 
The prediction should help our experts identify the translational potential of recent papers and indicate promising scientific areas and researchers for commercialization opportunities. 
The prediction model is based on the individual paper level and the prediction result will further be aggregated into researcher and scientific field levels. 

\subsubsection{Paper Metric} 
The goal of paper-level prediction is to indicate the probability of a paper being cited by different patent categories by using features of papers. 


\textbf{Input and Output Variables.} 
We collect the semantic content of papers and the structural relationship between them as input features, as suggested by our experts and literature~\cite{qian2021quantifying,qian2021geometric}. 
First, the semantic content of papers can provide insights into the topics covered in the paper, indicating the likelihood of it being cited in a patent and in which patent category. 
We utilize SPECTER~\cite{specter_cohan_2020} to embed the paper's title into a high-dimensional feature vector as its semantic content. 
Second, the citation relationship between papers can also provide helpful information as a paper citing other papers that have already been cited in patents may indicate that the focal paper may also be cited in patents. 
We thus create a citation graph between papers as the structural relationship. 
\wyf{Finally, we use CPC groups as the output variable to be predicted. } 
In addition, we also constrain the prediction targets based on domain knowledge. 
\wyf{First, we mainly focus on the prediction of recent papers since old papers are fully public knowledge and cannot be patented or further commercialized, even if it later turns out to have high commercial value.} 
Thus, we will focus on predicting the probability of receiving patent citations within $t$ years of publication. 
Here, we have set $t=5$ without loss of generality.
Second, we chose the top $50$ patent CPC groups in our two cases in Section~\ref{sec:06_Evaluation_CaseStudy} since the can account for the vast majority of patents (over 95\%) citing our target papers. 
We denote the set of $50$ patent CPC groups as $\mathbb{G}$. 
Thus, the goal is to investigate whether each paper published between 2001 and 2015 was cited by a patent from each of the top $50$ patent CPC groups that cited papers, within 5 years of its publication year. 

\textbf{Model Construction.} 
We aim to construct a model that can effectively use the above two input features to conduct prediction. 
As it is still an unclear and frontier problem about what important features contribute to paper-patent citation prediction, we here selected an end-to-end model without relying on sophisticated feature engineering. 
We applied Graph Convolutional Networks (GCNs)~\cite{kipf2017semi}, as they can effectively integrate both the semantic feature of each paper and the citation graph structure to learn meaningful representations of the papers. 

% To evaluate the potential translational impact of recently published papers on technology, relying solely on whether they receive patent citations is inadequate as they may not have had sufficient time to accrue citations. 
% For example, for papers published within the past year, it is crucial to predict their translational potential, as researchers can still patent their work within one year of publication. 
% After this period, the paper becomes fully public knowledge and cannot be patented or further commercialized, even if it later turns out to have high commercial value. 
% In such scenarios, a prediction model is required to predict the probability of receiving patent citations within $t$ years of publication. 
% Here, we have set $t=5$ without loss of generality.

% To exemplify the prediction model, we will use the case 1 as a running example. We investigated whether each paper published between 2001 and 2015 was cited by a patent from each of the top $50$ patent CPC groups that cited Northwestern's papers, within 5 years of its publication year. We denote the set of $50$ patent CPC groups as $\mathbb{G}$. The top $50$ CPC groups account for the vast majority of patents (over 95\%) citing Northwestern's papers. 

% To construct the prediction model, we employ both the semantic content of papers and the structural relationships between them. 
% First, we utilize SPECTER~\cite{specter_cohan_2020} to embed the paper's title into a high-dimensional feature vector, which encodes its semantic content. 
% Second, we create a citation graph, where each node represents a paper, and an undirected link connects two papers if one paper cites the other. 
% The two different data sources we use, the semantic embedding of paper titles and citation relationships between papers, can offer unique and valuable information for predictions~\cite{qian2021quantifying,qian2021geometric}. 
% The semantic embedding of a paper's title can provide insights into the topics covered in the paper, which can indicate the likelihood of it being cited in a patent and in which patent category. 
% On the other hand, the citation relationships between papers can also provide useful information as a paper citing other papers that have already been cited in patents may indicate that the focal paper may also be cited in patents. 
% Since both sources of information can contribute to better prediction performance, our aim is to leverage a machine learning model that can effectively combine both sources of data as inputs and be trained in an end-to-end manner without relying on sophisticated feature engineering with domain knowledge. 
% To this end, Graph Neural Networks (GNNs) are a natural choice for achieving this goal~\cite{bronstein2017geometric}, as they can effectively integrate both the features of each paper and the citation graph structure to learn meaningful representations of the papers. 
% GNNs have shown great success in various tasks, including classifications, and are thus a promising approach for our prediction model. 
% Specifically, we utilize Graph Convolutional Networks (GCNs)~\cite{kipf2017semi}, which are the canonical GNN models that have played a significant role in popularizing the GNN family of models.

Following the approach of the GCN~\cite{kipf2017semi}, we formulated our prediction tasks as a semi-supervised learning problem. 
As of the end of 2020, which is the most recent year in our system, we constructed the citation network between \YQ{Northwestern papers} published between 2001-2020, described by an adjacency matrix $A \in \mathbb{R}^{N \times N}$. 
Each paper is associated with an F-dimensional vector embedded from the SPECTER based on its title, which is arranged as a row of the feature matrix $X \in \mathbb{R}^{N \times F}$. 
For $N_{s}$ papers published between 2001-2015, for one patent CPC group $g$, we associated the paper with one of the $2$ classes, which is encoded into a 0-1 membership matrix $Y \in \mathbb{R}^{N_{s} \times 2}$ to indicate whether the paper is cited by patents from the CPC group $g$.

Our study applies the two-layer GCN~\cite{kipf2017semi}. Given the feature matrix X and the adjacency matrix A, the propagation rule is given by:

\begin{equation}
Z=f(X, A)=\mathrm{softmax}\left(\widehat{A} \mathrm{ReLU}\left(\widehat{A} X W^0\right) W^1\right)
\end{equation}

\noindent  where $W^{0}$ and $W^{1}$ are the weights connecting the layers of the GCN. The graph is encoded in
$\widehat{A}=\widetilde{D}^{-1/2}(A + I_{N})\widetilde{D}^{-1/2}$, where $I_{N}$ is the identity matrix, and $\widetilde{D}$ is a diagonal matrix with $\widetilde{D}_{ii} = 1 + \sum_{j}A_{ij}$. 
The softmax output $Z \in \mathbb{R}^{N \times 2}$ contains two probabilities for each paper, indicating the likelihood of the paper being cited by patents or not. 
The $\mathrm{softmax}$ and $\mathrm{ReLU}$ are threshold activation functions:

\begin{align}
\mathrm{ReLU}(x)_{i}=\max(x_{i},0)  \\
\mathrm{softmax}(x)_{i} = \frac{\exp(x_{i})}{\sum_{j} \exp(x_{j})}
\end{align}

\noindent where $x$ is a vector. 
For semi-supervised classification, we then evaluate the cross-entropy error over all the papers in the training set:

\begin{equation}
        \mathcal{L} = -\displaystyle\sum_{l\in \mathbb{N}_{T}}\displaystyle\sum_{c=1}^{2} Y_{lc} \, \ln{Z_{lc}},
    \label{eq:cross_entropy_error}
\end{equation}

\noindent where $\mathbb{N}_{T}$ is the set of papers in the training set. 
The weights of the neural network ($W^{0}$ and $W^{1}$) are trained using gradient descent to minimize the loss~$\mathcal{L}$. 

\textbf{Model Training, Validation, and Prediction.} 
We split the papers published between 2001-2014 into a training set (70\%) and a validation set (30\%), and use papers published in 2015 as the test set. 
For each paper published between $2016$-$2020$, we predict its likelihood of being cited by patents in CPC group $g$. 
We use the PyTorch Geometric implementation of GCN~\cite{Fey/Lenssen/2019} and follow the experimental setup in~\cite{kipf2017semi}. 
Our GCN model consists of two layers with $200$ epochs of training iterations, a learning rate of $0.01$, a dropout rate of $0.5$, and $16$ hidden units, which are model default parameters. 
Due to the class imbalance between papers that receive patent citations and those that do not, we evaluate the performance of our model using the AUC (Area Under the Curve) metric which is a common evaluation metric for imbalanced binary classification problems. 
Our final model is chosen from the epoch that produces the highest AUC score on the validation set. 
To assess the performance of the model, \wyf{we report its AUC on the test set in Section~\ref{sec:06_Evaluation_QuantitativeEvaluation}}.

To determine the likelihood of a paper $k$ published between $2016$-$2020$ being cited by patents in the CPC group $g$ within $5$ years of publication, we use the predicted probabilities in the softmax output matrix $Z$ obtained from the final model. 
To assess its relative importance within a specific range of papers (\eg, those within a research institution), we further convert its probability to a percentile, denoted as $\text{Patentability}_k^g$, which is a scalar ranging from 0 to 100.
% 
We iterate the above process on all the CPC groups in $\mathbb{G}$. 
% 
For a paper $k$ published between $2016$-$2020$, we take the average $\text{Patentability}(k,g)$ across CPC groups $g$ in $\mathbb{G}$ as $\text{Patentability}_k$ to further summarize its overall patentability. 

\subsubsection{Researcher Metric}
Based on the paper-level prediction, we examined the predicted $\text{Patentability}_k$ of a researcher's papers published from 2016 to 2020, and computed the average as their \textit{P-index}, which summarizes the predicted translational impact on patents of their research. 

The prediction result of a paper and researcher, together with other SciSci metrics, will be fed into the visualization system for exploratory analysis. 


==> sections/achieves/05_VisualDesign/05_VisualDesign.tex <==
\section{Visual Design}
\label{sec:05_VisualDesign} 
Guided by analytical tasks, we designed our visualization system with five coordinated views (Fig.~\ref{fig:system-ui}). 
Users will start from the \researcheroverviewview to choose a group of researchers~\wyf{(\textbf{\tasktypeoneshort1})}. 
The statistics and detailed individual information of these researchers will be summarized in the \researcherstatisticsview~\wyf{(\textbf{\tasktypeoneshort2})}. 
They can further narrow down researchers of interest based on demographic information (\eg, female researchers) or by choosing a specific researcher. 
The \innovationview will summarize \wyf{the interplay of science and technology} with more details~\wyf{(\textbf{\tasktypetwoshort1})}. 
First, the \interplayview visualizes the citation relationship between papers and patents. 
Users can explore science and technology fields from different LODs. 
Second, two sets of timelines are presented to show the evolution of science and technology respectively~\wyf{(\textbf{\tasktypetwoshort2})}. 
Finally, users can gain more context information in the \technologyinspectionview (with assignee distribution and patent topics) and \scienceinspectionview (with statistics and paper list)~\wyf{(\textbf{\tasktypetwoshort3})}. 
In addition to historical summarization, the system also provides the prediction results for users to identify potential inventors and inventions in multiple views (\ie, \researcheroverviewview, \researcherstatisticsview, \innovationview, and \scienceinspectionview)~\wyf{(\textbf{\tasktypethreeshort1})}. 


\subsection{\wyf{Researcher Overview View}}
\label{sec:05_VisualDesign_Researcher_Overview_View} 
The \researcheroverviewview \wyf{(Fig.~\ref{fig:system-ui}-A)} summarizes all researchers in terms of their \wyf{science and technology performance (\textbf{\tasktypeoneshort1})}. 

\textit{Description}: 
All the researchers are projected into a scatter plot. 
Users can specify two attributes of interest to visualize the distribution. 
Each circle represents a researcher, with opacity encoding the \textit{P-index} introduced in Section~\ref{sec:04_DataAnalysis}. 
We use a contour map to show areas with different densities, with darker regions having more researchers. 
Users can select a region and explore other views for more details. 
% All the researchers are summarized into a scatter plot with two modes. 
% In the dimension reduction mode, they are projected via t-SNE based on a set of measures proposed by our experts: \wyf{xx, xx, xx, xx, and the number of inventions (optional)}. 
% To provide a more explicit analysis of specific dimensions, 
% We also provide a two-dimension mode, allowing experts to specify two attributes of interest to learn the distribution. 
% In both modes, each circle represents a researcher, with its opacity encoding the \textit{P-index} introduced in Section~\ref{sec:04_DataAnalysis_ResearcherMetric}. 
% We also apply a contour map to reveal regions with different densities. 
% The darker the area, the denser number of researchers in this region. 

% \textit{Interaction}: 
% Users can select a region of interest and go to other views for detailed analysis. 
% Users can select a region of interest to highlight them in both two modes and go to other views for detailed analysis.  

\textit{Justification}: 
Given multiple researcher metrics, we first presented a dimension reduction mode to our experts to cluster researchers with multiple SciSci metrics. 
Although they agreed that it could identify clusters with multiple similar metrics, they could not quickly get the semantic meaning of the cluster. 
Thus, we use the current version that could allow them to customize two metrics of interest to project the researchers. 
% Thus, we also provided a simple version that could allow them to customize two metrics of interest to project the researchers. 


\subsection{\wyf{Researcher Statistics View}} 
\label{sec:05_VisualDesign_Researcher_Statistics_View} 
This view summarizes statistics and detailed researcher information of the selected group from \researcheroverviewview (\textbf{\tasktypeoneshort2}). 

\textit{Description}: 
The selected researchers' information is shown from two aspects.  
First, to show the semantic meaning of the selected group, we use bar charts to summarize the demographic information histograms to show the distribution of a set of SciSci metrics introduced in Seciton~\ref{sec:04_DataAnalysis}~\wyf{(Fig.~\ref{}-?)}. 
Second, researcher cards show detailed information such as affiliations per researcher~\wyf{(Fig.~\ref{}-?)}, which can be ranked by different SciSci metrics. 

\textit{Interaction}: 
Users can narrow down to select a group or individual of interest and go to the right three views to learn his/her details. 
% Two filtering approaches are provided. 
% First, users can select one or multiple attributes in the demographics bar charts to narrow down the interested researcher groups. 
% The other statistics charts, the researcher list, and the right three views will then be updated. 
% Second, users can also select a researcher and go to the right three views to learn his/her details. 

\textit{Justification}: 
At first, we only provided the statistics of selected researchers. 
During the design iteration, the experts specifically emphasized the importance of tracing individuals in their usage scenario, which can help them quickly locate interested researchers.  
Thus, we added the researcher list as another mode. 
% After iterations with our experts, they mentioned that in addition to the macro level summary, the micro level is also quite important in their usage scenario which can help them trace individual researchers of interest. 


\begin{figure*} [!htb]
 \centering 
 % \vspace{-0.5cm}
 \includegraphics[width=\linewidth]{figures/system-ui-20230330.png}
 % \vspace{-0.45cm} 
 \caption{The system UI of \systemname. 
The \researcheroverviewview (A) and \researcherstatisticsview (B) are for individual-level analysis (\tasktypeoneshort). 
The \innovationview (C) shows the detailed interplay between science and technology (\tasktypetwoshort, \tasktypethreeshort). 
The \technologyinspectionview (D) and \scienceinspectionview (E) provide additional contextual information about patents and papers (\tasktypeoneshort, \tasktypethreeshort).
 } 
 % \vspace{-0.5cm} 
 \label{fig:system-ui}
\end{figure*}


\subsection{\wyf{Innovation View}} 
\label{sec:05_VisualDesign_Innovation_View} 
The \innovationview \wyf{(Fig.~\ref{}-?)} is the primary visual component that enables users to explore the \wyf{interplay} between science (papers) and technology (patents). 
It consists of two parts: 
(1) the \interplayview visualizes the citation relation between papers and patents in a scalable manner~\wyf{(\tasktypetwoshort1)}. 
(2) two groups of \fieldtimeline show the temporal evolution of different fields in papers and patents, respectively~\wyf{(\tasktypetwoshort2)}. 

\subsubsection{\wyf{Interplay Graph}}
\label{sec:05_VisualDesign_Innovation_View_Interplay_Graph} 
The \interplayview shows \wyf{the citation linkage from patents to papers}, which supports exploring from different LODs \wyf{(\tasktypetwoshort1)}. 

\textit{Description}: 
it consists of three components, namely, \papermatrix, \patenttreemap, and \citationflow. 
The design of the \interplayview follows the idea of the compound graph~\cite{beck2017taxonomy}. 
Each node aggregates a group of papers or patents and thus makes it scalable to visualize a citation graph with large size. 
\wyf{The layout also follows the metaphor of a tree, where the \papermatrix represents the crown of a tree, the \citationflow is the trunk, and the \patenttreemap is the root. }
We have retained the top four levels (L0 to L3) from MAG, where L0 denotes broad fields such as \textit{computer science} and \textit{biology} and L2, L3, and L4 correspond to increasingly specific subfields. 
The \wyf{\textbf{Paper Matrix}} summarizes all papers from the science field and patent citation aspects. 
Each column represents a paper field with a blue circle on top of it showing the patent citation diversity of this field: \wyf{$diversity = -\sum_{i=1}^{n}P(x_i)logP(x_i)$}, where $i$ represent patent categories. 

Each row represents \wyf{different patent citation ranges}. 
\wyf{The lower the row, the higher the patent citation range these papers have.}  
For each cell, we provide two modes (\ie, folded mode and unfolded mode) to compare paper cells in two granularities. 
In the folded mode, \wyf{the color of the circle} represents the category of paper fields (based on Research Areas in Web of Science~\cite{wos}). 
The size of the circle encodes the average patent citation, and the opacity represents the number of papers in each cell. 
% glyph
The unfolded mode uses a glyph to summarize the statistics of papers \wyf{in terms of SciSci metrics, namely, xx, xx, xx, xx, xx, and xx}. 
The glyph is equally divided radially by six axes. 
Each axis represents the distribution of this metric. 
All the metrics are normalized globally to [0, 1] to support cross-glyph comparison. 
The radar area in the center represents the median value of each metric over this paper cell group. 

The \wyf{\textbf{Patent Icicle Plot}} uses an upturned icicle plot~\cite{kruskal1983icicle} to summarize the patent categories from a three-level hierarchy: CPC section, CPC subsection, and CPC group~\cite{cpcscheme}. 
Each rectangle represents a patent category with length encoding the number of patents in that category. 
The height of the rectangle is uniform across three levels. 

The \wyf{\textbf{Citation Flow}} visualizes citations from patents to papers. 
The flows will start from the \patenttreemap \wyf{(\ie, the ``tree root'')} and first converge at each paper field in the bottom of the \papermatrix 
Next, flows in each paper field will diffluence to each paper cell, \wyf{just like the ``tree branch''}. 
The width of the flow encodes the number of patent citations from a patent category (\eg, a rectangle in the \patenttreemap) to a paper cell. 
\wyf{The thicker the flow, the heavier the patent category relies on papers in the cell.} 
The color of the flow encodes the type: dark brown encodes the historical data, and light brown encodes the prediction result as \wyf{newly fledged trunk}. 
 
\wyf{We also apply a set of optimization approaches to make the flow aesthetically pleasing with fewer crossings. 
First, we reposition the paper fields in the \papermatrix. 
We iterate all field pairs and calculate their cosine similarity of patent citation so that two paper fields with similar patent citations will be paired together. 
This step is inspired by our experts' domain knowledge that specific patent categories will rely on multiple paper fields, so such kind of grouping can reveal such dependence to some degree. 
Second, we rank the sum of the number of patent citations (\ie, flow width) of paper field pairs in descending order and assign paper field pairs from the center to the left or right, which makes the \wyf{``tree''} visually balanced with \wyf{thick trunks} in the center. 
} 

\begin{figure} [!htb]
 \centering 
%  \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figures/interplay-graph-design-20230329.png}
%  \vspace{-0.5cm}
 \caption{The visual design of \interplayview. It consists of three components: Paper Matrix, Patent Icicle Plot, and Citation Flow. 
 } 
%  \vspace{-0.4cm}
 \label{fig:visual-design}
\end{figure}

\textit{Interaction}: 
A set of interactions are supported as follows: 
\begin{itemize}[leftmargin=10pt,topsep=1pt,itemsep=1px]
    % 1. hover & click
    \item \textbf{Hover and click to show more information.} 
    % 1-1. 点击paper cell, 展开/隐藏glyph和flow
    First, users can click each paper cell to switch between the above-mentioned folded and unfolded modes. 
    When the unfolded mode (\ie, glyph) is selected, corresponding patent citation flows will also be highlighted to show the patent categories that cite papers in this cell. 
    % 1-2. hover cpc: 显示cpc名字
    Second, in the \patenttreemap, users can hover each rectangle in the \patenttreemap to examine its CPC code and name. 
    % 1-3. 点击cpc rect: 高亮 flow， timeline，和右上角 
    Third, they can also click specific rectangles to highlight the citation flow to learn what kind of science is used by this patent category. 
    The patent assignee distribution and patent content wordle in the \technologyinspectionview will be updated to summarize this chosen patent category. 
    The corresponding chosen paper and patent timelines will also be highlighted and put on the top. 

    % 2. Zoom in paper/patent fields
    \item \textbf{Switch different levels in paper and patent fields.} 
    % 2-1. 点击Paper field展开
    For paper fields, users can click a specific paper field name to switch the paper fields between general disciplines and detailed topics. 
    % 2-2. 点击cpc field加号展开
    For the patent category, users can click the expand button on the left of each CPC level to zoom in to the next detailed level and click the patent level to return back to the upper level. 
    % 2-3. cpc field右键扩展: 解决scalability问题（flow太细）
    They can also right-click a rectangle of a patent category to expand the icicle plot to this level. It is useful when the experts want to check the detailed usage of a specific patent category, especially when the number of patents in this category is small compared with other categories. 
\end{itemize}
% 6. 框选左边一群人或一个人，中间更新。但是field位置是global的，为了减少cognitive load.
% 7. filter flows

\textit{Justification}: 
We have discussed a set of alternatives with our experts during the design process. 
At first, we started from the raw paper-patent citation network, where each node represented an individual paper or patent. 
Yet, the scalability of this graph becomes worse when the number of nodes becomes larger. 
Moreover, the experts mentioned that compared with the individual level, the field-level citation relation would be more meaningful to trace the development of different fields.  
% Second, given a large-scale citation graph between papers and patents, showing individual-level paper-patent citations becomes difficult and meaningless to trace the high-level citation pattern (\eg, citation linkages between fields). 
Thus, we tried a symmetrical compound graph, where each node encodes a paper or patent field. 
The experts suggested that the positions of papers and patents were not equal. 
They were more concerned with the paper side and wanted to learn how science enabled different patent categories. 
Specifically, they wished to compare papers in terms of the number of patent citations, \wyf{so that they could obtain which papers were heavily used by patents and compare differences between papers with diverse patent citations}. 
We first tried adding a histogram on top of each paper field and let experts brush papers based on patent citations. 
However, the experts felt the interaction is tedious and hard to compare among paper groups. 
Thus, we distributed the papers along the y-axis based on patent citation ranges and used the tree metaphor to combine both historical and prediction paper-patent citations coherently. 
\wyf{xxxxxxxxxxxxxxxxxx.}
% justification: 
% 0. paper和patent并不是完全对等的。Paper更重要
    % -> visual不一样；zoom-in交互也不一样（paper L0和L1之间不需要有层级关系；且这个是不可扩展的-L1种类太多了+不同L1 topic会出现在多个L0中，所以在L1层依旧可以看到跨学科合作）
% 1. 为什么不visualize individual paper network? (check之前的design Sketch和meeting notes)
    % abstract from single nodes to groups of nodes and make the visualization more scalable 
    % 配图：fluxflow那个设计。最多hold几百个node；还有ben那个设计也是；
    % 配图：metapbor树冠树干树根结构图
% 2. 圆形？
% 3. flow: matrix? dynamic network那个survey。专家觉得还是node-link更intuitive 
% Y-axis justification: 很重要，metaphor。一开始只做了paper_field -> patent field的对称的BPgraph，但是专家反馈2边并不是平等的。他们更重视the broad impact of science, which should put more data ink to it.  
% We unfold all papers in each field to different ro
% As it is important to distinguish papers in terms of patent citation, we calculate 
% paperMatrix: folded和unfolded mode的维度选择：不断跟专家迭代的结果


\subsubsection{\wyf{Field Timeline}}
\label{sec:05_VisualDesign_Innovation_View_Interplay_Graph} 
% 1. paper timeline: patent_citation_Call的百分比
Two groups of horizon charts are designed to compactly reveal the temporal evolution of different fields in science and technology \wyf{(\tasktypetwoshort2)}. 

\textit{Description}: 
Each paper or patent field is represented by a horizon graph. 
The chart is an improvement of an area chart that shows multiple attributes in a space-saving way. 
The x-axis is the timeline. 
The y-axis represents the proportion of papers or patents in each field in each year. 
The original area chart is partitioned into several bands horizontally with the same y-range. 
The saturation of the area encodes the y-value range. 
The darker the color, the higher the value. 
The bands are then shited and overlapped in this uniformed y-range. 
The scale of each horizon chart is independent, aiming to  show the temporal change of each field clearly. 

\textit{Interaction}: 
Two time sliders are provided to select period of interest and update the \interplayview and others. 

\textit{Justification}: 
The integration of temporal dimension has experienced several iterations with our experts. 
We first considered three versions of dynamic graphs to intergrate time dimension.
One is a timeline design~\cite{burch2011parallel}, where the x-axis is the timeline and the y-axis represents the paper or patent field node~\wyf{(Fig.~\ref{??})}. 
However, our experts felt that the time is the secondary important information dimension. 
They first would like to have an overview of all periods and then optionally choose to zoom in one period of interest. 
Thus, we proposed the second one which is a matrix design~\cite{burch2013matrix} and the temporal trend is embedded into each cell~\wyf{(Fig.~\ref{??})}. 
The experts felt difficult to understand the matrix and preferred the node link design which is more intuitive to study the citation relation. 
In the third compond node-link design~\wyf{(Fig.~\ref{??})}, we first link nodes to temporal charts and then show the citation relation. 
Nevertheless, it is not scalable to display all temporal charts in the graph and will distory the layout of the node link diagram. 
Thus, we finally put the timeline above the \interplayview as the secondary supplementary information. 

% 1. 一开始考虑的是dynamic graph，但是专家觉得这个是二级重要的信息，相比于时间，他们更希望首先看清楚citation likage。所以整个设计就以graph为主
% 2. compond graph有很多画法，例如matrix，直接embed timeline到node。但是again，他们提到这个是二级重要信息，更希望以更加直观的方式展现


\subsection{\wyf{Technology and Science Inspection}} 
\label{sec:05_VisualDesign_Technology_and_Science_Inspection} 
The \technologyinspectionview and \scienceinspectionview presents other aspects of patents and papers to understand the \wyf{interplay} in depth (\wyf{\tasktypetwoshort}3). 

\textit{Description}: 
The \technologyinspectionview includes a two-level sunburst showing the proportion of assignees and a word cloud in the center showing the keywords of the selected patents. 
The \scienceinspectionview shows a list of \wyf{SciSci metrics} at the paper level, such as the patentability prediction score. 
It also provides a paper list with different ranking criteria. 

\textit{Interaction}: 
In the \technologyinspectionview, a slider is provided to show the top k assignees in terms of the number of patents. 
Users can hover over each sector to learn the full name and number of patents of the assignee. 
They can also click an assignee of interest to learn how patents in this assignee consume science in the \interplayview. 
In the \scienceinspectionview, users can brush papers with high patentability prediction scores and the prediction flow will be presented in the \interplayview. 

\textit{Justification}: 
At first, we use three bar charts to show the assignee distribution: one showing the proportion of company and university assignees, the other two showing the top five assignees in each category. 
The experts felt the second level is limited to showing a small number of assignees and they expected to learn more assignees. 
Thus, we applied a sunburst with a slider to show the top k assignees. 


% \subsection{\wyf{Science Inspection View}} 
% \label{sec:05_VisualDesign_Science_Inspection_View} 
% Suggestion: 
% 五个指标的顺序需要调整，调整为一下顺序：Patentability Prediction Distribution (chart颜色跟其他不一样); Science Citations Distribution; Disruption Distribution; Novelty Distribution; Patent Citation Distribution;    另外需要告诉用户指标好的方向，citations是数值越大越好，disruption是数值越大越好，novelty这里是数值！越小！越好，patent citations是越大越好，Patentability Prediction是越大越好







% Justification: check 
% 1. Notion的system UI history
% 2. Design部分有早起的圆形设计

==> sections/achieves/06_Evaluation/06_Evaluation_20230331_0950.tex <==
\section{Evaluation}
\label{sec:06_Evaluation} 
\wyf{We evaluate \systemname through two case studies and interviews with experts, as well as a quantitative study of the prediction model.}  

\subsection{Model Eavaluation} 
Due to the class imbalance between papers that receive patent citations and those that do not, we evaluate the performance of our model using the AUC (Area Under the Curve) metric. 
% , which is a common evaluation metric for imbalanced binary classification problems. 
Our final model is chosen from the epoch that produces the highest AUC score on the validation set. 
We evaluate the model by presenting their prediction performance and scalability in the two datasets used in two case studies (Section~\ref{sec:06_Evaluation_CaseStudy}). 

\begin{itemize}[leftmargin=10pt,topsep=1pt,itemsep=0px]
    \item \textbf{AUC}. We present the AUC results on the test set across CPC groups by CPC section in Fig.~\ref{fig:case1_case2_auc}. The overall prediction performance is good and remains robust across different CPC groups. 
    \item \textbf{Scalability}. The time complexity of GCN has been demonstrated to be linear in the number of graph edges and can scale to millions of edges according to Kipf and Welling in~\cite{kipf2017semi}. In our two cases, the training time per epoch is less than 10 seconds with CPU-only implementations. We also run the codes in parallel for different CPC groups to accelerate the prediction process. Moreover, the prediction model is pre-executed and does not impact the visualization system in real time. 
\end{itemize}
    
\begin{figure}[H]
  \centering
  \begin{subfigure}[b]{0.45\columnwidth}
  	\centering
  	\includegraphics[width=\textwidth]{figures/06_Evaluation/case1_auc.pdf}
  	% \caption{}
  	\label{fig:case1_auc}
  \end{subfigure}%
  \hfill%
  % \\%
  \begin{subfigure}[b]{0.45\columnwidth}
  	\centering
  	\includegraphics[width=\textwidth]{figures/06_Evaluation/case2_auc.pdf}
  	% \caption{} 
  	\label{fig:case2_auc}
  \end{subfigure}%
  \subfigsCaption{This figure shows the prediction performance (AUC) on the test set for two case studies. The average AUC and its 95\% confidence interval are reported for each case and CPC section, based on the performance across CPC groups within that section. The dashed lines at 0.5 indicate the baseline performance of random guesses.
  Overall, the results demonstrate good performance for our prediction tasks.
  }
  \label{fig:case1_case2_auc}
\end{figure} 


\subsection{Case Study} 
\label{sec:06_Evaluation_CaseStudy} 
We invited our experts 
% in Section~\ref{sec:03_Background_ProblemFormulation} 
to freely explore \systemname. 
We summarize their findings through two case studies to demonstrate our system. 
% We then summarized observations and formed into two cases to fully demonstrate our system. 

\subsubsection{New Opportunities for University Innovation} 
\label{sec:06_Evaluation_CaseStudy_Case1_NU} 
We pilot the system with a premier research university and focus on $461$ faculty who have at least one paper that has been cited by a patent. 
This case study demonstrates how \systemname enables our experts (\ea and \eb) to uncover new innovation opportunities and facilitate knowledge transfer for researchers. 
% \wyf{We pilot the system with a premier research institution, helping its institution leaders to extract new insights for innovation.} 
% We focus on $461$ faculty who have at least one paper that has been cited by a patent and their 37K papers which enables us focusing on researchers whose papers have impact on patents. 

\wyf{\textbf{Overview of the innovation landscape}}. 
Upon loading the data from \universityname, the experts started from the \citationflow (Fig.~\wyf{\ref{??}-C1}), finding 
\textit{Material science}, \textit{biology}, and \textit{chemistry}, as  the three predominant disciplines whose knowledge has spurred inventions across many categories such as \textit{A} (\textit{``Human Necessities''}) and \textit{C} (\textit{``Chemistry; Metallurgy''}). 
Highlighting \textit{C}, the experts noticed that in addition to \textit{chemistry}, it also cited papers from \textit{material science} and \textit{biology}. 
\wyf{\textit{``This patent category seems to be built on interdisciplinary scientific knowledge.''}} 
% \wyf{\textit{``This patent category seems to be built on interdisciplinary knowledge sourced from multiple broad scientific fields.''}} 
% 
% 
The experts also noticed that the diversity of the paper-patent citation is quite high in \textit{material science} (Fig.~\wyf{\ref{??}-C2}). 
Clicking to zoom in, it had enabled at least six patent major categories. 
Noticeing \textit{C} is an emerging category (Fig.~\wyf{\ref{??}-C4}), they expanded it to get more detailed CPC categories. 
% C08J
The most emerging technology lay in \textit{C08J} (\textit{General Processes Of Compounding}). 
It mostly consumed knowledge in \textit{nanotechnology} and \textit{composite material} (Fig.~\wyf{\ref{fig:case1}-B1}), indicating they were dominant research topics in this university that contributed to this emerging patent category. 
\textit{Nanotechnology} remained popular, while \textit{composite material} surged at the beginning of 21 century (Fig.~\wyf{\ref{??}-C5}). 
The expert also noticed that this patent category heavily relied on papers with high patent citations (Fig.~\wyf{\ref{??}-B2}) in \textit{nanotechnology}, signifying their importance in technology development. 
Thus, the experts chose this paper cell and found that the top-citation papers were related to \textit{polymer nanocomposites} (Fig.~\wyf{\ref{??}-xx}). 
% ~\cite{ramanathan2008functionalized, kim2010waterproof}  
To get more aspects about \textit{C08J}, the experts went to the \technologyinspectionview (Fig.~\wyf{\ref{fig:system-ui}-D}). 
Unexpectedly, the largest university assignee is KFUPM
% ~\footnote{http://www.kfupm.edu.sa/Default.aspx} 
(a university in Saudi Arabia, Fig.~\wyf{\ref{??}-xx}) instead of \universityname itself, and the patents were related to \textit{polymer}, \textit{graphene}, and \textit{energy} (Fig.~\wyf{\ref{fig:system-ui}-D1}). 
Choosing this assignee and they found it just started citing papers in \universityname in recent years. 
The experts never realized this before, \wyf{\textit{``in most cases, we expect our university to be the largest university assignee citing our papers. 
So this finding is rather unexpected. Maybe there's collaboration opportunities with KFUPM, especially in \textit{nanotechnology}.''}} 


\begin{figure} [tb]
 \centering 
%  \vspace{-0.2cm}
 \includegraphics[width=\linewidth]{figures/case-1-20230330.png}
%  \vspace{-0.5cm}
 \caption{
    \wyf{The paper-patent citation relationship and innovation insights of a group of researchers in a university. 
    (A) The \interplayview shows their predominant science fields and citation relations at different paper field levels.  
    (B) For a particular patent group (C08J), it mostly consumed knowledge in \textit{nanotechnology} and \textit{composite material}. 
    }
 } 
%  \vspace{-0.4cm}
 \label{fig:case1}
\end{figure}


\wyf{\textbf{Uncover the talents}}. 
After getting an overview of the knowledge consumption of \universityname, our experts also aimed to identify innovation opportunities and faculty with untapped commercialization potential. 
Thus, they examined the \researcheroverviewview (Fig.~\wyf{\ref{fig:system-ui}-A}), focusing on invention disclosures (as the y-axis) and patent-cited papers (as the x-axis). 
% Thus, they turned to the \researcheroverviewview (Fig.~\wyf{\ref{??}-xx}) and selected the number of invention disclosures and \wyf{the number of papers cited by patents} to distribute the researchers.  
At the bottom (Fig.~\wyf{\ref{fig:system-ui}-A1}), a line of researchers immediately caught their eyes: 
they themselves had no invention disclosures, while their papers had been frequently cited by other patents. 
\wyf{The experts were excited, ``their work may have high unrealized potential for commercialization.''} 
Further analysis in the \researcherstatisticsview (Fig.~\wyf{\ref{fig:system-ui}-B1}) revealed most of them were full professors in medical school. 
% Choosing these researchers and going to the \researcherstatisticsview, the experts noticed most of them were full professors from the medical school (Fig.~\wyf{\ref{??}-xx}). 
They chose the medical school to learn more details. 
Most of their papers were in the \textit{biology} (Fig.~\wyf{\ref{fig:case1}-A1}), and surprisingly, company patents dominate the assignee types (Fig.~\wyf{\ref{fig:case1}-B3}). 
\wyf{\textit{``Compared with university assignees, patents with company assignees signify that their research has a tangible impact on the industry and imply a significant potential for patenting their own research findings.''}} 

Next, the experts sought to identify future research directions for this group of faculty in the medical school to foster their knowledge transfer to technology. 
% Next, the experts wanted to know future research directions this group of researchers in the medical school should focus on. 
% This can help with decision-making at the school level to encourage these faculty to transfer knowledge to more technological advancement. 
Thus, they filtered recent papers with high patentability prediction scores. 
After exploring paper fields from different levels, the experts discovered unexpected misalignments in specific fields. 
Despite limited historical citations, recent \textit{medicine} papers showed significant patent citation potential in the future (Fig.~\wyf{\ref{fig:case1}-A1}).  
% Many recent papers in the \textit{medicine} field have presented a larger potential to be cited by patents in the future, regardless of their minor historical citation compared with other fields. 
More specifically, \textit{intensive care medicine} and \textit{physical medicine and rehabilitation} emerged as areas warranting increased focus (Fig.~\wyf{\ref{fig:case1}-A2}). 
Choosing papers in \textit{intensive care medicine} with no current patent citation and ranking based on the prediction score, \wyf{the experts noticed recent papers with high prediction scores were about nanomedicine and drug allergy (Fig.~\wyf{\ref{??}-xx}),  
% ~\cite{hagemeyer2020nanomedicine, sanchez2019controversies} 
and planned to discuss the patenting potential with the faculty authors}. 

In addition to scientific directions and specific papers, the experts are also interested in identifying researchers with high commercialization potential. 
Thus, they returned to the \researcherstatisticsview and ranked the previously selected researchers by P-index. 
They quickly noticed the second faculty (Fig.~\wyf{\ref{fig:system-ui}-B2}) had a noticeably high P-index and was the only female faculty among top P-index researchers. 
She had no inventions while having many papers cited by other patents. 
From the \interplayview (Fig.~\wyf{\ref{fig:case1}-A3}), most of her papers cited by patents were in \textit{cell biology}. 
From the patent category (Fig.~\wyf{\ref{fig:system-ui}-C4}), \textit{C12N} 
\wyf{(\textit{Microorganisms Or Enzymes; Mutation Or Genetic Engineering})} 
were increasingly citing her papers, where most assignees were companies, particularly \textit{Immatics Biotechnologies}
% ~\footnote{https://immatics.com/} 
from Germany. 
\wyf{Subsequent discussions with this faculty revealed that she used to attend conferences in Germany, which could potentially explain how this company became interested in her research.}
In addition, the other two universities were two top university assignees (Fig.~\wyf{\ref{fig:case1}-B5}). 
% , instead of \universityname. 
\wyf{``We ourselves are not aware of her work...''}
The experts further queried the prediction results and found that in addition to \textit{cell biology}, some works in \textit{genetics} also had high potential to be cited by patent in the future. 
The experts got detailed paper information
% ~\cite{vodo2018striate, maruthappu2019loss, boyden2016dominant} 
in the \scienceinspectionview and talked with this faculty. 
After the conversation, she promptly submitted new invention disclosures to the university TTO in two weeks, \wyf{in which the content was related to paper topics in the high prediction score studies}. 

\wyf{The case demonstrates how to use \systemname to find innovation opportunities in research institutions.}

\begin{figure*} [!htb]
 \centering 
 % \vspace{-0.5cm}
 \includegraphics[width=\linewidth]{figures/case-2-20230330.png}
 % \vspace{-0.45cm} 
 \caption{
    \wyf{Innovation Insights from Case 2 (VIS/HCI community).} 
 } 
 % \vspace{-0.5cm} 
 \label{fig:case2}
\end{figure*}

\subsubsection{\wyf{Innovation Insights in VIS and HCI Communities}} 
\label{sec:06_Evaluation_CaseStudy_Case2_VIS} 
In this case, our experts (\ec and \ed) used \wyf{\textit{visualization} and \textit{human computer interaction}} as example fields to explore the impact of science on technology.
\wyf{Specifically, we extracted papers from six major journals and fourteen leading conferences (please refer to supplementary material) in these fields. 
We then work with our experts to narrow authors who had published at least \wyf{ten} papers in these venues as active researchers. 
% Next, we examined all papers published by these authors and retained only those who had at least five papers cited by patents. 
Our final dataset included $2016$ researchers and a total of 129K papers authored by them. 
}
% We summarized interesting findings from our experts as follows. 
% case 2: vis
% 需要讲清楚人数刷选的标准：researcher人数（参考ACSeeker / SciSci是否有些metrice可以衡量一个人是否在一个领域活跃？） @yifan (好像说过是根据paper发布数量等刷选人数的)
% 还要claim，假设我们站在2020年末。这样的话，2020年发表的paper还有可能被transfer成未来的topic 

\noindent \wyf{\textbf{What is the next science ``fruit'' to mature?}}
The experts first zoomed in on the paper topic of \textit{human computer interaction} and then \textit{visualization}. 
From the paper field timeline (Fig.~\wyf{\ref{??}-xx}), two topics quickly caught their eyes: \textit{mixed reality} and \textit{3d computer graphics}. 
They also noticed that these two topics were paired together in the \interplayview (Fig.~\wyf{\ref{??}-xx}). 
It indicated that they were always cited by similar patent categories. 
The experts then filtered recent papers with high prediction scores. 
Unexpectedly, although other fields (\eg, \textit{image porocessing} and \textit{real time rendering}) had occupied the majority historically, \textit{mixed reality} was the top paper field with the highest prediction score papers recently. 
Highlighting the paper cell in this field and they found the prediction flows were linked to various CPC categories (\eg, \textit{G06F} (\textit{Electric Digital Data Processing}) and \textit{G06T} (\textit{Image Data Processing Or Generation})). 
\wyf{\textit{``All these confirmed that `mixed reality' is a potential science topic that will enable new patents in the future in various industries and professions. 
We should pay more attention to this science direction.''}}

From the patent aspects (Fig.~\wyf{\ref{??}-xx}), the experts noticed that \textit{A} (\textit{Human Necessities}) is a rising category. 
Zooming in \textit{A}, they found that \textit{volume rendering} was the most applied science topic (Fig.~\wyf{\ref{??}-xx}) and was primarily used in \textit{A61B} (\textit{Diagnosis; Surgery}). 
Highlighting \textit{A61B} and in the \technologyinspectionview (Fig.~\wyf{\ref{??}-xx}), the experts confirmed that these patents were related to medical devices. 
Moreover, most patent assignees were companies, indicating that scientific knowledge was most likely transformed into actual products. 
Curious about what papers were highly cited by patents, the experts clicked the paper cell in the last row (Fig.~\wyf{\ref{??}-xx}). 
Unexpectedly, the highly cited papers in this emerging patent category were not new (published in the early 2000s). 
\wyf{\textit{``Interesting, even over ten years later, papers in `volume rendering' have still been used by new patents. These high-impact papers may have a long-lasting impact on emerging technologies and can even become seminal works in this field.''}} 

\noindent \wyf{\textbf{Does technology increasingly rely on older scientific knowledge?}} 
Curious about the findings in the last story, the experts return to the \textit{human computer interaction} field and filtered patent application years based on three ranges in the early, mid, and end of 2001 to 2020. 
\wyf{In recent years (\eg, [2019, 2020] (Fig.~\wyf{\ref{??}-xx}) and [2015, 2016] (Fig.~\wyf{\ref{??}-xx}))}, the patent citation of old and new papers was diverse. 
They either cited new paper fields (\ie, \textit{visualization} and \textit{wearable computer}), or cited fallen fields many years ago (\textit{ubiquitous computing} and \textit{user interface}). 
However, when time went back ten more years ago, patents tended to cite more new paper fields at that time (\eg, [2010, 2011] (Fig.~\wyf{\ref{??}-xx}) and [2004, 2005] (Fig.~\wyf{\ref{??}-xx})). 
\textit{``This finding is aligned with our hypothesis that new technologies are increasingly relying on older scientific knowledge. 
\wyf{We observe a growing time lag between citing patents and cited papers, which warrants a dedicated study to understand the possible mechanisms that drive this phenomenon.''} 
% \wyf{We observe a growing time lag between citing patents and cited papers, which warrants a dedicated study to understand the possible mechanisms that drive this phenomenon.''}
}

\noindent \wyf{\textbf{What paper characteristics are associated with its use in technology?}} 
The experts also explored the differences between highly patent-cited papers and other papers, \wyf{with the aim of identifying distinctive characteristics that could aid in their differentiation.}. 
To incorporate more papers and get a general finding, the experts zoomed out and used the most prominent field, \textit{computer vision}, as an illustrative example. 
% To incorporate more papers and get a general finding, the experts zoomed out to the paper field level 1. 
% They chose the most prominent field, \textit{computer vision}, as an example. 
After controlling for publication years by studying papers in the same period \wyf{(\eg, [2011, 2014], [2005, 2008], and [2001, 2004])}, they found similar results (Fig.~\wyf{\ref{??}-xx})). 
Generally, science citations and novelty have positive relationships with patent citations, whereas disruption has a negative relationship with patent citations.  
% Generally, the more patent citations these papers had, the more novel these papers were, the more science citation these papers got, and the less disruptive these papers were. 
\wyf{\textit{``These results are consistent with our recent findings. 
Papers receiving high citations within the scientific community are often associated with a higher impact on downstream innovations, including patents~\cite{yin2022public}. 
% This can be explained by the fact that these papers can provide a strong foundation of established knowledge and insights in a particular field. 
% Subsequent inventors frequently reference these papers in their own work, building upon or applying the established knowledge to further advance the field. 
Furthermore, the results raise new research questions regarding the connections between novelty, disruption, and patent citations. 
This visual comparison of different dimensions facilitated a more streamlined and effective comparison process.''}}

\wyf{The case used three stories to demonstrate the usefulness of our system in confirming existing results and uncovering new insights in science and technology.} 


\subsection{\wyf{Expert Interview}} 
\label{sec:06_Evaluation_ExpertInterview} 
We first collected feedback from experts in Section~\ref{sec:03_Background_ProblemFormulation}. 
We also interviewed six external experts who used \systemname for the first time. 
\newea and \neweb are innovation managers in the technology transfer office (TTO) of a university. 
\newec and \newed are researchers in SciSci who work on the public usage of science. 
Although the target users of \systemname are SciSci researchers and policymakers in research institutions, the dataset in case 2 we use may also interest visualization researchers. 
Thus, we also included two vis researchers (\newee and \newef) who have at least three-year visualization expertise. 

\textbf{Procedure.} 
Each interview with each external expert lasted around 90 minutes. 
We first briefly introduced the background of our project, including the analytical tasks and data sources we use. 
Second, we use case 1 in Section~\ref{sec:06_Evaluation_CaseStudy_Case1_NU} to demonstrate the system workflow and visual encodings. 
Third, they were asked to freely explore the system in a think-aloud manner. 
Finally, we had a semi-structured expert interview. 
We took notes about their comments and findings during the process. 
The feedback from two groups of experts is summarized below. 

\textbf{System Workflow.} 
All experts appreciated the clear workflow. 
\ea commented, \textit{``the system entry which starts from scientific fields or researchers of interest is exactly what we (TTO) expect to analyze the innovation opportunities.''} 
They were able to learn and follow the system logic quickly, from researcher identification to paper-patent interaction exploration. 
We also observed different exploration focuses along with experts from different fields. 
In addition to those from the TTO who focused on researchers and their research fields, 
experts from SciSci and vis fields were more interested in directly starting from scientific fields. 
As \newec mentioned, \textit{``we are more interested in the general findings over some scientific field.''}
Nevertheless, they agreed that the current workflow was able to meet different needs using filtering conditions provided by the system. 

\textbf{SciSci Metrics and Prediction Model.} 
% 1. vis人觉得很有用，team_size和novelty之类的measure以前不知道
% 2. TTO: particularly like the P-index, 可以直接帮助他们Identify人；improvement：对model内部原理很好奇。希望可以找到一些有用的measure来indicate if a researcher is with high P-index (commercialization potential)
The experts all showed interest in these metrics. 
Those from TTO were particularly interested in the \textit{P-index} obtained from the prediction model. 
\textit{``This is a much more straightforward way for me to locate faculty with high commercialization potential, I indeed came across a lot of researchers that I didn't notice previously,''} \neweb was excited. 
\ea also suggested making the prediction model more transparent to help them understand the mechanism behind the prediction. 
\newee and \newef found several metrics such as \textit{team size} and \textit{novelty} very interesting, \textit{``these metrics help us look at papers from new perspectives except paper citation.''} 

\textbf{Visualization and Interactions.} 
% 1. graph design: easy to understand (TTO + VIS) ; 交互很直观
% 2. hot area timeline: very useful (TTO)
All the experts thought the visual components in the system were intuitive and satisfied all the analytical tasks. 
Many of them appreciated the \researcheroverviewview, the \interplayview, and the \technologyinspectionview. 
\eb said, \textit{``I can directly choose a group of interest in this scatterplot. 
It's straightforward.''} 
For the \interplayview, \ea and \newef mentioned that although it would take more time to understand the encoding, it finally became very useful and intuitive after he figured out the meaning. 
\newec though the y-axis in the paper matrix was great that she could locate papers with high patent citations more quickly. 
\neweb and \newee liked the \technologyinspectionview. 
\textit{``It's really beautiful, ''} suggested by \neweb, \textit{``but it would be more interesting if I could check the linkages between these assignees, for example, via the similarity of paper-patent citing behaviors. 
It can help us to find missing opportunities in licensing with the industry.''} 
\newec and \newef liked the glyph design, ``it makes the comparison between paper groups much easier. But it would be great if somewhere could tell me the meaning of dimensions such as labels.''
\ea also mentioned the timeline as important, \textit{``it's useful to check recent hot areas as a temporal indicator to the innovation.''} 

\textbf{Suggestions.} 
The experts also provided valuable suggestions. 
In addition to universities and research fields, \ed also wanted to filter researchers at the regional and state level to obtain a higher level comparison of different geo regions. 
\eb would like the system to show information step-by-step to avoid information being overwhelming. 
\ea suggested using text analysis to learn more details about paper-patent citation, such as strong citation (\eg, cite the core knowledge in the paper) and weak citation (\eg, just cite a paper for the background part). 
% suggestions 
% 1. 如果先点了中间的论文类别，比如biology，那左边的人到更新到只做这些papers的人吗，问题是比如说我想看Northwestern有biology paper的人。当然了，这个情节和先在左边选school很像。但是也不太一样，比如说想找出Northwestern做cancer research的人该如何实现呢？
% 2. yifan说想看到visualization跟哪些别的paper field同时出现在同一类patent。这个需要跨topic 层级。因为现在的top%8一般都是cs领域内部的topic。别的topic有但是在很后面
% 3. As a benchmarking tool: scalable to other universities and make comparisons. 
